Generalized Neural Collapse for a Large Number of Classes

Neural collapse provides an elegant mathematical characterization of learned last layer representations (a.k.a. features) and classifier weights in deep classification models. Such results not only provide insights but also motivate new techniques for improving practical deep models. However, most of the existing empirical and theoretical studies in neural collapse focus on the case that the number of classes is small relative to the dimension of the feature space. This paper extends neural collapse to cases where the number of classes are much larger than the dimension of feature space, which broadly occur for language models, retrieval systems, and face recognition applications. We show that the features and classifier exhibit a generalized neural collapse phenomenon, where the minimum one-vs-rest margins is maximized.We provide empirical study to verify the occurrence of generalized neural collapse in practical deep neural networks. Moreover, we provide theoretical study to show that the generalized neural collapse provably occurs under unconstrained feature model with spherical constraint, under certain technical conditions on feature dimension and number of classes.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}
Over the past decade, deep learning algorithms have achieved remarkable progress across numerous machine learning tasks and have significantly enhanced the state-of-the-art in many practical applications ranging from computer vision, natural language processing and retrieval systems. Despite their tremendous success, there is still no comprehensive understanding of the feature characterization learned from deep neural networks (DNNs). Consequently, they are often criticized for being treated as opaque "black boxes". In recent years, several studies have uncovered an intriguing phenomenon called  \emph{Neural Collapse} (\NC) regarding the last-layer features and classifier of DNNs during the terminal phase of training. Specifically, the \emph{Neural Collapse} phenomenon can be summarized as following properties of the last-layer features and classifier:
\begin{itemize}[leftmargin=0.3in,topsep=0.2em,itemsep=0.11em]
    \item \textbf{ \emph{Variability Collapse}:} the distance of any pairs of features from the same classes converges to zero. 
    \item \textbf{ \emph{Convergence to Simplex ETF}:} the class-mean of features from different classes exhibits a Simplex Equiangular Tight Frame (ETF) strcuture such that the distance among any pairs of features from the different classes are equal and maximal.
    \item  \textbf{\emph{Convergence to Self-duality}:} the linear classifiers converge to their corresponding class-mean of features.
    \item \textbf{ \emph{Simple Decision Rule}:} the last-layer classifier works according to Nearest Class-Center decision rule.
\end{itemize}
Neural collapse provides a mathematically elegant characterization of learned representations or features in deep learning based classification models regardless of network architectures, datasets and optimization algorithms.
However, most of the existing empirical and theoretical studies in neural collapse focus on the case that the number of classes is small relative to the dimension of the feature space. 
In practice, there are many cases where the number of classes can be extremely large. 
\begin{itemize}
    \item Contrastive representation learning, where each training data instance can be regarded as one class.
    \item Masked language modeling, where the number of classes is equal to the vocabulary size.
    \item Retrieval systems where the number of classes is equal to the number of the documents.
    \item Face identification where the number of classes is equal to the number of person identity in the system. 
\end{itemize}
In such cases, it is usually infeasible to have a feature dimension commensurate with the number of classes, which means that the condition for the existence of \NC\ is not met. In this work, we aim to understanding the configurations of the learned features and last-layer classifier when the feature dimension is smaller than the number of classes

Here we provide a novel analysis of geometry of learned representations, which can cover the case that the number of classes is larger than the dimension of the feature space. 
Our analysis is based on examining the separation of classifier weight vectors associated with different classes.
Our result sheds light on the property of the learned representations, which may have practical implications. 

\zz{meeting on March 23:
\begin{itemize}
    \item Study within-class collapse for new loss function (classifiers being the class-mean features) for $K>d$.
    \item Under this setting: study the global solutions, the distribution of the class-mean features for $K>d$. Maybe also add the results for $d = 2$.
    \item Experiments: \begin{itemize}
    \item Verify theory and justify the value of the new loss (performance improvement): experiments under standard loss and the new loss on CIFAR-100. Metric: within-class collapse, max-mean angles? Performance quality (accuracies, convergence). Fine-tuning: new loss gives better OOD performance.
    \item Assignment for each class: $d=2, K =4$ (standard loss (different distribution of classifiers) and new loss); and large $K$ (different random initialization givens different results? if so, any method to find a good one; setting?)
    \end{itemize}
\end{itemize}
}

\newpage
\zz{Story for submission, if we can only prove within-class collapse for the regularized version. [Add proof.] 
\begin{itemize}
    \item Whole story is the focus on the analysis for neural collapse and class separation when $K> d$. 
    \item Motivation 1: use simple experimental results to show a very slow convergence of alignment between classifier and class-mean features. Motivated by this fact, we set the classifier as class-mean features, and prove its within-class collapse. Therefore, we simply focus on the setting of one sample per class in the following analysis. 
    \item Motivation 2: even with setting the classifier as class-mean features, use a simple experimental result to show that different classes could have different lengths of features. We then normalize the features to the unit sphere. Do we observe better performance with constraints on the sphere?
    \item Now the problem becomes
    \[
\min_{\u_1,\ldots,\u_K\in\Sp^{d-1} } \sum_{k=1}^K \log\left( 1 + \sum_{k'\neq k} \exp(\alpha - \alpha (\langle \u_k, \u_{k'} \rangle))   \right).
\]
\pw{This should be} 
    \[
\min_{\u_1,\ldots,\u_K\in\Sp^{d-1} } \sum_{k=1}^K \log\left( 1 + \sum_{k'\neq k} \exp(\alpha \langle \u_k, \u_{k'} \rangle - \alpha)   \right).
\]
Then present the results for this problem: 
\begin{itemize}
    \item Universal result:     Since LogSumExp is an approximation of the maximum function, if we ignore the constant $\exp(1)$\footnote{Or, can we argue that when the maximum is a constant (\ie, $1$), LogSumExp approximates in some sense the second maximum?}, this is saying that approximately the minimum pairwise angle between rows of $\W^*$ is maximized. More precisely, 
        \begin{multline}
            \frac{\log 2}{\alpha} + \sum_{k}\max_{k' \ne k} \left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2} \right\rangle
            \le
           \frac{1}{\alpha} \log\left( \exp(1) + \sum_{k' \ne k} \exp \left(\alpha\left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2} \right\rangle\right) \right)\\
            \le 
            \frac{\log (\exp(2)+k-1)}{\alpha} + \sum_k\max_{k' \ne k} \left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2} \right\rangle
        \end{multline}
        Please unify all the notations. 
        \jz{there is some mistakes in the above range}
        \item When $K\rightarrow \infty$, the minimizer is uniformly distributed over the sphere.
        \item The solution $\U = \begin{bmatrix}\u_1 & \cdots & \u_K \end{bmatrix}$ always forms a tight frame, i.e., $\U\U^\top \sim I_d$. Could we approve this?
        \item How $\alpha$ affect the convergence, if not the global minimum? Example: $d 2$, fix $K-2$ points and only optimize the other two points. As Peng said, compute the Hessian and gradient. Plot a figure. 
        \item $d+2\le K\le 2d$: could we prove $
\max_{k\neq k'} \langle \u_k, \u_{k'} \rangle = 0$ is achieved by CE solution?
\item $d=2$, could we approve that the minimizer is uniformly distributed over the sphere?
\item Results for MSE loss?
\end{itemize}
\item Experiments: see above. 
\end{itemize}
}
\zz{If we set the classifier as the class-mean features, is the new loss equivalent to contrastive loss used in self-supervised learning?}

\zz{CE loss in supervised classification: 
\begin{align*}
& CE_{supervised} = \sum_{k}\log\paren{ \sum_{k'} \frac{\exp\paren{\vw_{k'}^\top\vh_k}}{\exp\paren{\vw_k^\top\vh_k}}    
} \\
& CE_{unsupervised-contrastive} = \sum_{k}\log\paren{ \sum_{k'} \frac{\exp\paren{\vw_{k'}^\top\vw_k}}{\exp\paren{\vw_k^\top\vh_k}} 
} , \ \vw_k = f(\vx), \vw_{k'} = f(\vx^-), \vh_k = f(\vx^+)   
\end{align*}
could we prove the equivalence between each other?
}

 \jz{To show the lower and upper bound for the cross-entropy loss using the nearest class, let first show the lower and upper bound for the logsumexp function. Before starting proof, let denote $\vx^k=\left[x^k_1, x^k_2, \cdots, x^k_K\right]^\top\in\reals^K$, We can have
 \begin{align*}
     \exp{(\alpha x^k_k)} + \max_{i\neq k}\exp{(\alpha x^k_i)} <\sum_{i=1}^K \exp{(\alpha x^k_i)}&\le \exp{(\alpha x^k_k)} + (K-1)\max_{i\neq k}\exp{(\alpha x^k_i)}\\
     \log\paren{\exp{(\alpha x^k_k)} + \max_{i\neq k}\exp{(\alpha x^k_i)}} <\log\paren{\sum_{i=1}^K \exp{(\alpha x^k_i)}}&\le \log\paren{\exp{(\alpha x^k_k)} + (K-1)\max_{i\neq k}\exp{(\alpha x^k_i)}}\\
     \alpha\max_{i\neq k}x_i^k+\log\paren{\exp{(\alpha x_k^k-\alpha\max_{i\neq k}x_i^k)}+1}<\log\paren{\sum_{i=1}^K \exp{(\alpha x^k_i)}}&\le \alpha\max_{i\neq k}x_i^k+\log\paren{\exp{(\alpha x_k^k-\alpha\max_{i\neq k}x_i^k)}+K-1}
 \end{align*}
 If we denote $x_i^k = 1 - \langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_i}{\|\w_{i}\|_2}\rangle \in [0,2]$ and $x_k^k=0$, then the lower bound:
 \begin{align*}
    \alpha\max_{i\neq k}x_i^k+\log\paren{\exp{(\alpha x_k^k-\alpha\max_{i\neq k}x_i^k)}+1} > \alpha\max_{i\neq k}x_i^k + \log\paren{\exp{(-2\alpha)}+1} 
 \end{align*},
similarly the upper bound is:
 \begin{align*}
    \alpha\max_{i\neq k}x_i^k+\log\paren{\exp{(\alpha x_k^k-\alpha\max_{i\neq k}x_i^k)}+K-1} < \alpha\max_{i\neq k}x_i^k + \log\paren{\exp{(2\alpha)}+K-1} 
 \end{align*}.
 Therefore, we can have the range for the cross-entropy loss:
 \begin{align*}
     \max_{i\neq k}x_i^k+\frac{1}{\alpha}\log\paren{\exp{(-2\alpha)}+1}&<\frac{1}{\alpha}\log\paren{\sum_{i=1}^K \exp{(\alpha x^k_i)}}\\
     &\le  \max_{i\neq k}x_i^k + \frac{1}{\alpha}\log\paren{\exp{(2\alpha)}+K-1}
 \end{align*}
}

\jz{alternative problem:
\[
\min_{\theta_1,\ldots,\theta_K\in[0, 2\pi) } \sum_{k=1}^K \log\left( 1 + \sum_{k'\neq k} \exp(\alpha - \alpha (\cos(\theta_k-\theta_{k'})))   \right).
\]
}


\section{The arrangement problem}

\subsection{Class Separation with MSE and CE Losses}

For the classification of $K$-classes, we can consider a simple case where the training samples of each class are balanced(i.e. $n_1 = n_2 = \cdots = n_K = n$). We assume that all biases $\{\b_i\}_{i=1}^d $ of the last layer classifier are zero. Deep networks are very complex to analyze due to their nonlinear interactions. To make the analysis simpler, we adopt the unconstrained feature model (UFM) following previous works \cite{??} and treat the last-layer features as free optimization variables. This is based on the idea that modern deep networks are often overparameterized and can approximate any continuous function. By doing so, we simplify the nonlinear interactions across layers. Consider the unconstrained feature model,
% \begin{align}\label{eq:obj}
%      \min_{\W , \H} & f(\W,\H):= \frac{1}{N}\sum_{k=1}^K \sum_{i=1}^{n} {\mc L} \paren{\W\h_{k,i},\y_k } + \frac{\lambda_{\W} }{2} \norm{\W}{F}^2 
%      + \frac{\lambda_{\H} }{2} \norm{\H}{F}^2.
% \end{align}
\begin{align}\label{eq:obj}
     \min_{\W , \H} & f(\W,\H):= \frac{1}{N}\sum_{k=1}^K \sum_{i=1}^{n} {\mc L} \paren{\W\h_{k,i},\y_k }, \ \st \|\vw_k\| = 1, \|\vh_{k,i}\| = 1.
\end{align}
In above, $\W = [\w_1, \ldots, \w_K] ^\top \in \RR^{K \times d}$, $\H = [\H_1, \ldots, \H_K] \in \RR^{d \times N}$, $\H_k = [\h_{k, 1}, \ldots, \h_{k, n}] \in \RR^{d \times n}$, where $d$ is the dimension of the feature space and $N = K \times n$ is the total number of training examples. 

Let $(\W^*, \H^*)$ be a global solution to \eqref{eq:obj}, and define $\h_{k}^* \doteq \sum_{i=1}^n \h_{k,i}^*$.

\begin{conjecture}[Within-class Collapsing]\label{conj:within-class-collapsing}
All features within each class are identical, \ie, for each $k=1, \ldots, K$ we have $\h_{k,i}^* \equiv \h_{k}^*, \forall i$.
\end{conjecture}

\begin{conjecture}[Self-duality]\label{conj:self-duality}
    The mean feature of each class is proportional to its corresponding classifier weight, \ie, for each $k=1, \ldots, K$ we have $\h_k^* =  \w_k^*$ for some $\alpha > 0$ independent of $k$. 
\end{conjecture}

\begin{conjecture}[Uniformity]\label{conj:uniform}
\end{conjecture}

% \begin{conjecture}[Equal norm]\label{conj:equal-norm}
%     The norm of classifier weight for all classes are equal, i.e., $\|\w_k\|_2 \equiv \beta$ for some $\beta > 0$ independent of $k$.\footnote{Not sure if this actually holds and we may get some clue from simulations; if not, maybe we can modify the definition of UFM to have it as a constraint.} This seems holds for relatively large $K$, but may not hold when $K$ is too large. We can check this from experiments. \zz{new conjecture: if a minimizer does not have equal-norm rows, its normalized version is still a global minimizer.} 
% \end{conjecture}



%\zz{Maybe we can study the loss functions of the following form \begin{align*}
% {\mc L} \paren{\W\h_{k},\y_k } = g\left( \sum_{i\neq k} h(\w_i^\top \h_k - \w_k^\top \h_k)  \right)
% \end{align*} where $g$ and $h$ are increasing functions. CE is a special function corresponding to a particular choice for $g$ and $h$. Feel like as long as $g$ and $h$ are increasing functions, then minimizing it with weight decay or sphere constraints will lead to self-duality. We may look at the gradient and Hessian.
% \begin{align*}
% &{\mc L} \paren{(\W+\Delta_{\W})(\h_{k}+d_{h_k}),\y_k } \\
% & = g\left( \sum_{i\neq k} h\left((\w_i+ \delta_{\w_i})^\top (\h_k + \delta_{h_k}) - (\w_k + \delta_{\w_k})^\top (\h_k + \delta_{\h_k})\right)  \right)\\
% & = g\left( \sum_{i\neq k} h\left( \w_i^\top \h_k -\w_k^\top \h_k +  \delta_{\w_i}^\top \h_k  + \w_i^\top \delta_{\h_k} + \delta_{\w_i}^\top \delta_{\h_k}  +  \delta_{\w_k}^\top \h_k  + \w_k^\top \delta_{\h_k} + \delta_{\w_k}^\top \delta_{\h_k}   \right)  \right) \\
% & = g\Big( \sum_{i\neq k} h\left( \w_i^\top \h_k -\w_k^\top \h_k   \right) + h'\left( \w_i^\top \h_k -\w_k^\top \h_k   \right) \cdot \left(   \delta_{\w_i}^\top \h_k  + \w_i^\top \delta_{\h_k} + \delta_{\w_i}^\top \delta_{\h_k}  +  \delta_{\w_k}^\top \h_k  + \w_k^\top \delta_{\h_k} + \delta_{\w_k}^\top \delta_{\h_k}   \right)\\
% & \qquad \qquad + \frac{h''\left( \w_i^\top \h_k -\w_k^\top \h_k   \right)}{2} \cdot \left(   \delta_{\w_i}^\top \h_k  + \w_i^\top \delta_{\h_k} + \delta_{\w_i}^\top \delta_{\h_k}  +  \delta_{\w_k}^\top \h_k  + \w_k^\top \delta_{\h_k} + \delta_{\w_k}^\top \delta_{\h_k}   \right)^2 + \text{higher order}
% \Big)
% \end{align*}
% }

\begin{proof} 





\paragraph{Different phenomena between $K\ge d$ and $K<d$}

\zz{Add a simplex experiment e.g., on CIFAR10, to show that when $d \le K-1$, the class-mean features and the classifier weight could have different length, and the ratio $\|\ol \vh_k\|/\|\vw_k\|$ also varies across different classes. Also for some losses, like the MSE loss, some classes may collapse to each other. Therefore, we restrict the features and classifier on the unit sphere, which is a common practice when the number of classes is large.}
\begin{figure} [!ht]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar100+_res18_d2_k30_fixdim_2.png}
         \caption{Visualization of features from the first 30 classes in CIFAR100 with $n = 500$ samples per class, with class-mean features and classifier weights. The network used is Resnet18, and the features and classifiers are found through optimizing the cross-entropy loss, where features are embedded in 2-dimensional space, i.e. $d = 2$.}
         \label{fig:features}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/feature_length.png}
         \caption{Comparison of the length of class-mean features and classifier weights among different classes in CIFAR10 when $d = 2 \leq K-1$. We use $\mathbf{l}_2$ norm of the features to represent their length, e.g. $\|\overline{\h}_k - \h_G\|_2$ is class-mean feature and $\|\w_k\|_2$ is classifier weight of class $k$. Notice that the class-mean features and the classifier weight could have different lengths, and the ratio $\|\overline{\h}_k - \h_G\|_2 / \|\w_k\|_2$ also varies across different classes.}
         \label{fig:feature_length}
     \end{subfigure}
        \caption{CIFAR100 Class Separation Experiments when $d = 2 \leq K-1$}
        \label{fig:Exp_d<K}
\end{figure}

\begin{figure} [!ht]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/distribution_K=30.png}
         \caption{Visualization of class-mean features and classifier weights of $30$ classes under unconstrained feature model with $n=5$ samples per class. The features and classifiers are found through optimizing the cross-entropy loss with weight decay, where features are embedded in 2-dimensional space, i.e. $d = 2$.}
         \label{fig:features}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/feature_length_K=30.png}
         \caption{Comparison of the length of class-mean features and classifier weights among different classes when $d = 2 \leq K-1$. We use $\mathbf{l}_2$ norm of the features to represent their length, e.g. $\|\overline{\h}_k \|_2$ is class-mean feature and $\|\w_k\|_2$ is classifier weight of class $k$. Notice that the class-mean features and the classifier weight could have different lengths, and the ratio $\|\overline{\h}_k\|_2 / \|\w_k\|_2$ also varies across different classes.}
         \label{fig:feature_length}
     \end{subfigure}
        \caption{Class Separation Experiments when $d = 2 \leq K-1$ under unconstrained feature models.}
        \label{fig:Exp_d<K}
\end{figure}


\begin{figure} [!ht]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/constrained_distribution_K=30.png}
         \caption{Visualization of class-mean features and classifier weights of $30$ classes under spherical constrained feature model with $n=5$ samples per class. The features and classifiers are found through optimizing the cross-entropy loss with temperature $\tau = 0.05$, where features are embedded in 2-dimensional space, i.e. $d = 2$.}
         \label{fig:Fix_W}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/constrained_feature_length_K=30.png}
         \caption{The length of classifier weights and class-mean features are equal. } 
         \label{fig:margin}
     \end{subfigure}
        \caption{Class Separation Experiments when $d = 2 \leq K-1$ under spherical constrained feature models.}   \label{fig:Margin}
\end{figure}

Based on the experiment on CIFAR10, we assume that both the features and the classifiers are normalized, i.e. $\|\h_{k,i}\|_2 = 1$, $\|\w_k\|_2 = 1$, for all $k \in [K]$ and all $i \in [n]$. Also we need to add a temperature parameter $\tau > 0$ to control the entropy of a distribution. As a result, we obtain a formulation under unit sphere constrains,
\begin{equation}
\label{eq:constrained_feature_model}
\begin{aligned}
    \min_{\W,\H} \quad & f(\W,\H) := \frac{1}{nK} \sum_{k = 1}^{K} \sum_{i= 1}^{n} L(\tau \W^{\top} \h_{k,i},\y_k) \\
    \st \quad & \|\vw_k\|_2 = 1, \ \|\vh_{k,i}\|_2 = 1.
\end{aligned}
\end{equation}
Regarding the Cross Entropy(CE) loss for vector $\z \in \mathbb{R}^K$,
\begin{equation}
    \mathcal{L}_{CE}(\z,\y_k) := -\log(\frac{\exp(z_k)}{\sum_{l = 1}^{K} \exp(z_l)}).
\end{equation}

\newpage
\begin{theorem}
    Consider the following optimization problem 
    \begin{equation}
\begin{aligned}
    \min_{\W,\H} \quad & f_\tau(\W,\H) :=  \sum_{k = 1}^{K}  \log\paren{\sum_{k'=1}^K \frac{\exp\paren{\tau\vw_{k'}^\top \vh_k}}{  \exp\paren{\tau\vw_{k}^\top \vh_k}  }  } \\
    \st \quad & \|\vw_k\|_2 = 1, \ \|\vh_{k}\|_2 = 1.
\end{aligned}
\label{eq:CE-sphere-one-sample}\end{equation}
When $\tau\rightarrow \infty$, the above problem converges to the following problem
    \begin{equation}
    \label{eq:min-max-one-sample}
\begin{aligned}
    \min_{\W,\H} \quad & \max_{k} \max_{k' \neq k} \langle \w_{k'} - \w_{k} , \h_k \rangle \\
    \st \quad & \|\vw_k\|_2 = 1, \ \|\vh_{k}\|_2 = 1.
\end{aligned}
\end{equation}
\end{theorem}
\begin{proof} \zz{Here is a rough outline:} First note that
\[
\sum_{k'=1}^K \frac{\exp\paren{\tau\vw_{k'}^\top \vh_k}}{  \exp\paren{\tau\vw_{k}^\top \vh_k}  } = 1 + \sum_{k'\neq k} \exp\paren{\tau (\vw_{k'} - \vw_k)^\top \vh_k }.
\]
Since $\log$ is an increasing function, when $\tau$ goes to $\infty$, minimizer of \eqref{eq:CE-sphere-one-sample} must satisfy $(\vw_{k'} - \vw_k)^\top \vh_k <0$. We can prove this by contradiction. Thus, in the following, we will only consider $(\mW,\mH)$ such that $(\vw_{k'} - \vw_k)^\top \vh_k <0, \forall k\neq k'$. Now, when $\tau \rightarrow \infty$, we have $\sum_{k'\neq k} \exp\paren{\tau (\vw_{k'} - \vw_k)^\top \vh_k }\rightarrow 0$, and hence
\[
\log\paren{ 1 + \sum_{k'\neq k} \exp\paren{\tau (\vw_{k'} - \vw_k)^\top \vh_k } } \rightarrow \sum_{k'\neq k} \exp\paren{\tau (\vw_{k'} - \vw_k)^\top \vh_k }, 
\]
which further implies that when $\tau \rightarrow \infty$,
\[
f_\tau(\W,\H) =  \sum_{k = 1}^{K}  \log\paren{\sum_{k'=1}^K \frac{\exp\paren{\tau\vw_{k'}^\top \vh_k}}{  \exp\paren{\tau\vw_{k}^\top \vh_k}  }  } \rightarrow \sum_{k}\sum_{k'\neq k} \exp\paren{\tau (\vw_{k'} - \vw_k)^\top \vh_k }.
\]
Hence, when $\tau \rightarrow \infty$, minimizing $f_\tau(\W,\H)$ is equivalent to minimizing 
\[
g_{\tau}(\W,\H)=\frac{1}{\tau}\log\paren{\sum_{k}\sum_{k'\neq k} \exp\paren{\tau (\vw_{k'} - \vw_k)^\top \vh_k }}.
\]
Note that the above involves LogSumExp function, which is a smooth approximation to the maximum function and converges to the maximum function when $\tau \rightarrow \infty$. In particular, we have
\[
 \max_{k,k'\in[K], k'\neq k} (\vw_{k'} - \vw_k)^\top \vh_k \le g_{\tau}(\W,\H) \le  \max_{k,k'\in[K], k'\neq k} (\vw_{k'} - \vw_k)^\top \vh_k + \frac{\log (K(K-1)) }{\tau},
\]
which further implies that
\[
g_{\tau}(\W,\H) \rightarrow  \max_{k,k'\in[K], k'\neq k} (\vw_{k'} - \vw_k)^\top \vh_k, \quad \text{as} \ \tau \rightarrow \infty. 
\]
\end{proof}

\begin{definition}
    \label{def:tammes}
    \textbf{(Tammes Problem).} The Tammes problem is a problem of finding the maximum possible minimum distance between a set of points arranged on the surface of a sphere. Suppose the vectors are $\{\vw_k \}_{k=1}^{K}$ and $\vw_k \in \mathbb{R}^d$, then the Tammes problem can be solved by optimizing,
    \begin{equation}
        \min_{\vw_k} \max_{k} \max_{k^{'} \neq k} \langle \vw_{k^{'}}, \vw_k \rangle , \quad \st \quad \|\vw_k\|_2 = 1.
    \end{equation}
    
\end{definition}

\begin{definition}
\label{def:max-margin-spherical-codes}
    \textbf{(Maximum Margin Spherical Codes Problem).} Suppose the vectors are $\{\vw_k \}_{k=1}^{K}$ and $\vw_k \in \mathbb{R}^d$, let $margin(\vw_k, \overline{\vw}_k)$ denote the distance between $\vw_k$ and the convex hull of all of the other vectors $ \overline{\vw}_k := \{ \vw_{k^{'}} \}_{k^{'} \neq k}^{K}$. Then Maximum Margin Spherical Codes Problem is hunting for the arrangement $\{ \vw_{k} \}_{k = 1}^{K}$ of points on the surface of the sphere that,
    \begin{equation}
        \max_{\vw_k} \min_{k} margin(\vw_k, \overline{\vw}_k), \quad \st \quad \|\vw_k\|_2 = 1.
    \end{equation}
\end{definition}

\begin{definition}
    \textbf{(Intersection Solution Set).} We define Intersection Solution Set as pairs of $(d, K)$ on which Tammes problem is equivalent to Maximum Margin Spherical Codes Problem. 
    \begin{equation}
        \mathbb{S} := \{(d,K) | \argmin_{\vw_k} \max_{k} \max_{k^{'} \neq k} \langle \vw_{k^{'}}, \vw_k \rangle = \argmax_{\vw_k} \min_{k} margin(\vw_k, \overline{\vw}_k), \vw_k \in \mathbb{R}^d, \forall k \in [K]\}
    \end{equation}
\end{definition}

\begin{theorem}
    \label{thm:GNC}
    \textbf{(Generalized Neural Collapse Under Sphere Constrains).} Suppose that the number of classes is larger than feature dimension plus one, i.e. $K > d + 1$, and the training labels are balanced in each class, i.e., $n = n_1 = \cdots =n_K$. If $\tau \rightarrow 0$, then optimizing problem \ref{eq:CE-sphere-all-sample} would lead to the following conclusion,
    \begin{itemize}
    \item \textbf{(GNC1) Within-class variability collapse:} All the features of the same class converge to their within-class feature mean, i.e., $\vh_{k,i} = \overline{\vh}_k, \ \forall \ i \in [n],\ k\in[K]$.
    \item \textbf{(GNC2) Convergence to maximum margin spherical codes: } $\W$ converges to solution of maximum margin spherical codes problem. Moreover, for $(d, K) \in \mathbb{S}$, $\W$ would converges to solution of Tammes problem. 
    \item \textbf{(GNC3) Convergence to self-duality:} Suppose $(d, K) \in \mathbb{S}$ and there is no rattlers for Tammes problem under such $(d,K)$, then the linear classifier would converge to their corresponding feature class-means, i.e., $\vw_k = \overline{\vh}_k, \ \forall \ k\in[K]$.
    \end{itemize}
\end{theorem}


Experiments 

\textbf{Setup for Network Architectures, Dataset, and Training.} CE loss/ ResNet18/ CIAFR100/ d=10/ Epoch200/ SGD/ Normalization/ $\tau = 0.05$.

\textbf{Metric for Measuring $\mathcal{GNC}$ During Network Training.} We measure $\mathcal{GNC}$ for the learned features and last-layer classifier weights based on \ref{thm:GNC}. We define the global mean and within-class mean of features $\{ \vh_{k,i}\}$ as,
\begin{equation}
    \vh_G = \frac{1}{nK} \sum_{ k =1}^{k} \sum_{i=1}^{n} \vh_{k,i}, \quad \overline{\vh}_k = \frac{1}{n} \sum_{i = 1}^{n} \vh_{k,i} \ (k \in [K])
\end{equation}

\begin{itemize}
\item \textbf{Within-class variability collapse.} The within-class and between-class covariance matrices are,
\[
\boldsymbol{\Sigma}_W := \frac{1}{nK} \sum_{ k =1}^{k} \sum_{i=1}^{n} \paren{\vh_{k,i} - \overline{\vh}_k} \paren{\vh_{k,i} - \overline{\vh}_k}^\top, \quad \boldsymbol{\Sigma}_B := \frac{1}{K} \sum_{k=1}^{K} \paren{\overline{\vh}_k - \vh_G}\paren{\overline{\vh}_k - \vh_G}^\top
\]
Thus, we quantify the within-class variability collapse via,
\begin{equation}
    \mathcal{NC}_1 := \frac{1}{K} \trace \paren {\boldsymbol{\Sigma}_{W} \boldsymbol{\Sigma}_B^{\dagger} }
\end{equation}
where $\boldsymbol{\Sigma}_B^{\dagger}$ denotes the pseudo inverse of $\boldsymbol{\Sigma}_B$.
\item \textbf{Convergence to maximum margin spherical codes.} Given feature dimension $d$ and number of classes $K$, we use Riemannian Gradient Descent on the constrained feature model to generate numerical solution to maximum margin spherical codes problem as $\A \in \mathbb{R}^{K \times d}$. For the learned classifier $\W \in \mathbb{R}^{K \times d}$, there is a permutation matrix $\P$ that $\A \approx \P \W$. So we quantify the closeness by,
\begin{equation}
    \mathcal{NC}_2 :=  \left\| \frac{\W^{\top} \W}{\|\W^{\top} \W\|_F} -  \frac{\A^{\top} \A}{\|\A^{\top} \A\|_F} \right\|_F
\end{equation}
\jc{It doesn't converge to 0 because our NC2 forget to consider rotation. Actually, $\A \approx \P \W \boldsymbol{R}$, where permutation matrix $\P \in \mathbb{R}^{K \times K}$, rotation matrix $\boldsymbol{R} \in \mathbb{R}^{d \times d}$. }

\item \textbf{Convergence to self-duality.} 
\begin{equation}
    \mathcal{NC}_3 :=  \frac{1}{K} \sum_{k =1}^{K} \paren{1 - \w_{k}^{\top} \vh_{k}}
\end{equation}

\end{itemize}


\begin{figure} [!ht]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/NC1.png}
         \caption{NC1.}
         \label{fig:NC1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/NC2.png}
         \caption{NC2. }
         \label{fig:NC2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/NC3.png}
         \caption{NC3.}
         \label{fig:NC2}
     \end{subfigure}
        \caption{CIFAR100 GNC Experiments when $d = 10 \leq K-1$}
        \label{fig:NC}
\end{figure}



\begin{theorem}
\jc{CE loss would converge to hardmax problem when temperature $\tau \rightarrow 0$. I rewrite it in all sample form because we need it to prove with-class collapse.}
    Consider the optimization problem \ref{eq:constrained_feature_model} under CE loss which is,
    \begin{equation}
\begin{aligned}
    \min_{\W,\H} \quad & f_\tau(\W,\H) := \sum_{i = 1}^{n} \sum_{k = 1}^{K}  \log\paren{\sum_{k'=1}^K \exp\paren{\langle \vw_{k'} - \vw_k, \vh_{k,i} \rangle / \tau} } \\
    \st \quad & \|\vw_k\|_2 = 1, \ \|\vh_{k}\|_2 = 1.
\end{aligned}
\label{eq:CE-sphere-all-sample}\end{equation}
When $\tau\rightarrow 0$, the above problem converges to the following problem
    \begin{equation}
    \label{eq:min-max-all-sample}
\begin{aligned}
    \min_{\W,\H} \quad & \max_{i} \max_{k} \max_{k' \neq k} \langle \w_{k'} - \w_{k} , \h_{k,i} \rangle \\
    \st \quad & \|\vw_k\|_2 = 1, \ \|\vh_{k,i}\|_2 = 1.
\end{aligned}
\end{equation}
We call the problem \ref{eq:min-max-all-sample} as "HardMax Problem" since it replaces the SoftMax function in CE loss with the hard max function.
\end{theorem}

\begin{proof} First note that
\[
\sum_{k'=1}^K \exp\paren{\langle \vw_{k'} - \vw_k, \vh_{k,i} \rangle / \tau}= 1 + \sum_{k'\neq k} \exp\paren{(\vw_{k'} - \vw_k)^\top \vh_{k,i} /\tau }.
\]
Since $\log$ is an increasing function, when $\tau$ goes to $\infty$, minimizer of \eqref{eq:CE-sphere-all-sample} must satisfy $(\vw_{k'} - \vw_k)^\top \vh_{k,i} <0$. We can prove this by contradiction. Thus, in the following, we will only consider $(\mW,\mH)$ such that $(\vw_{k'} - \vw_k)^\top \vh_{k,i} <0, \forall k\neq k'$. Now, when $\tau \rightarrow \infty$, we have $\sum_{k'\neq k} \exp\paren{\tau (\vw_{k'} - \vw_k)^\top \vh_{k,i} }\rightarrow 0$, and hence
\[
\log\paren{ 1 + \sum_{k'\neq k} \exp\paren{ (\vw_{k'} - \vw_k)^\top \vh_{k,i} /\tau } } \rightarrow \sum_{k'\neq k} \exp\paren{\tau (\vw_{k'} - \vw_k)^\top \vh_{k,i} }, 
\]
which further implies that when $\tau \rightarrow 0$,
\[
f_\tau(\W,\H) =  \sum_{i = 1}^{n} \sum_{k = 1}^{K}  \log\paren{\sum_{k'=1}^K \exp\paren{\langle \vw_{k'} - \vw_k, \vh_{k,i} \rangle / \tau} } \rightarrow \sum_{i = 1}^{n} \sum_{k = 1}^{K}  \sum_{k'\neq k}^{K} \exp\paren{(\vw_{k'} - \vw_k)^\top \vh_{k,i} / \tau}.
\]
Hence, when $\tau \rightarrow 0$, minimizing $f_\tau(\W,\H)$ is equivalent to minimizing 
\[
g_{\tau}(\W,\H)=\tau \log\paren{\sum_{i} \sum_{k}\sum_{k'\neq k} \exp\paren{(\vw_{k'} - \vw_k)^\top \vh_{k,i} /\tau }}.
\]
Note that the above involves LogSumExp function, which is a smooth approximation to the maximum function and converges to the maximum function when $\tau \rightarrow 0$. In particular, we have
\[
 \max_{i \in [n],k,k'\in[K], k'\neq k} (\vw_{k'} - \vw_k)^\top \vh_k \le g_{\tau}(\W,\H) \le  \max_{i \in [n],k,k'\in[K], k'\neq k} (\vw_{k'} - \vw_k)^\top \vh_k + \log (nK(K-1)) \tau,
\]
which further implies that
\[
g_{\tau}(\W,\H) \rightarrow  \max_{i \in [n],k,k'\in[K], k'\neq k} (\vw_{k'} - \vw_k)^\top \vh_{k,i}, \quad \text{as} \ \tau \rightarrow 0. 
\]
\end{proof}

\begin{theorem}
    \jc{Prove within-class collapse by fixing $\vw_k$ and optimizing $\vh_{k,i}$ under the hardmax problem.} Optimizing the "HardMax Problem" of \ref{eq:min-max-all-sample} would lead to within-class variability collapse, indicating that all features of the same class $\vh_{k,i}$ would converge to their within-class feature mean. It can be expressed as,
    \begin{equation}
        \vh_{k,i}^{*} = \vh_{k,j}^{*} =  \vh_{k}^{*}, \quad \forall i,j \in [n]
    \end{equation}
\end{theorem}

\begin{proof}
Consider the "HardMax Problem" \ref{eq:min-max-all-sample},
\[
\begin{aligned}
\min_{\W,\H} \quad & \max_{i} \max_{k} \max_{k' \neq k} \langle \w_{k'} - \w_{k} , \h_{k,i} \rangle \\
\st \quad & \|\vw_k\|_2 = 1, \ \|\vh_{k,i}\|_2 = 1.
\end{aligned}
\]
To find the optimal $\vh_{k,i}^*$, firstly we can fix all weight vectors $\{\vw_k\}_{k = 1}^{K}$. Then for a specific class k, the optimizing problem can be decoupled as,
\begin{equation}
    \min_{\vh_{k,i}} \quad \max_{i} \max_{k^{'} \neq k} \langle \vw_{k^{'}} - \vw_{k}, \vh_{k,i} \rangle, \quad \st \quad \ \|\vh_{k,i}\|_2 = 1.
\end{equation}
Define a optimal feature vector $\vh_{k,i}^*$ as,
\[
\vh_{k,i}^* = \argmin_{\vh_{k,i}}  \quad  \max_{k^{'} \neq k} \langle \vw_{k^{'}} - \vw_{k}, \vh_{k,i} \rangle
\]
Define another optimal feature vector $\vh_{k,j}^*$ as,
\[
\vh_{k,j}^* = \argmin_{\vh_{k,j}} \quad  \max_{k^{'} \neq k} \langle \vw_{k^{'}} - \vw_{k}, \vh_{k,j} \rangle
\]
For a specific class k, define $\{ \vh_k^*, \b_k^* \}$ as the optimal solution of max-min margin for one-vs-all separation problem \ref{eq:max_min_margin}. According to Lemma \ref{lemma:max_min_separation_margin}, we have
\[
 \vh_{k,i}^{*} = \vh_{k}^{*}, \quad \vh_{k,j}^{*} = \vh_{k}^{*} \quad \forall i,j \in[n].
\]
which is,
\[
\vh_{k,i}^{*} = \vh_{k,j}^{*} = \vh_{k}^{*} \quad \forall i,j \in[n].
\]

    

\end{proof}

\begin{lemma}
\label{lemma:max_min_separation_margin}
Assume the classifier weights $\{ \vw_{k} \}_{k = 1}^{K}$ are fixed, for a specific $k$, consider optimizing,
\begin{equation}
    \min_{\vh} \quad  \max_{j \neq k}\langle \vw_{j} - \vw_k, \vh \rangle, \quad \st \quad  \ \|\vh\|_2 = 1, \forall k.
\label{eq:fix_w_find_h}
\end{equation}
Consider a binary classification problem that can be solved by finding a separating hyperplane. Suppose the data points are $\x_{j} = \vw_{j} - \vw_k$, then take a single data point $\x_{k} = \0$ as one class with label $y_k = +1$, and take all other data points $\{\x_{j} \}_{j \neq k}^{K}$ as the other class with labels $y_{j} = -1$. To find a hyperplane $\vh^{\top} \x + \b = \0$ that can separate these two classes with the largest margin, we optimize:
\begin{equation}
    \max_{\vh,\b} \quad \min_{j} margin(\x_{j}),\quad \st \quad  \ \|\vh\|_2 = 1, \forall k. 
    \label{eq:max_min_margin}
\end{equation}
where $margin(x_{j})$ is defined as the distance of $\x_j$ to the separating hyperplane. 

If the optimal solution of max-min margin for one-vs-all separation problem \ref{eq:max_min_margin} is $\{ \vh^*, \b^*\}$, then $\vh^*$ is the solution of problem \ref{eq:fix_w_find_h}.
\end{lemma}

\begin{proof}
We define a hyperplane as $\vh^{\top} \x + \b = \0$, where $\vh$ is a unit norm vector that is orthogonal to the hyperplane with the direction pointing to the class with label $+1$, i.e. $\x_k = \0$. So the $margin(x_{k})$ can be defined as,
\begin{equation}
    margin(\x_{j}) := \y_j(\vh^{\top} \x_j + \b) = \left\{
    \begin{aligned}
        \b \quad \quad ,& \quad j = k \\
        -(\vh^{\top} \x_{j} + \b) ,& \quad j \neq k \\
    \end{aligned}
    \right.
\end{equation}
Then problem \ref{eq:max_min_margin} is,
\begin{equation}
    \max_{\vh,\b} \quad \min_{j} \y_j(\vh^{\top} \x_{j} + \b),\quad \st \quad  \ \|\vh\|_2 = 1, \forall k. 
\end{equation}
To find a optimal $b_k^*$, we need to guarantee that $margin(\x_k)$ equals $min_{j \neq k} margin(x_j)$. Notice $\b$ is the distance of $\x_k = \0$ to the hyperplane so the optimal $\b^*$ should satisfy,
\begin{equation}
    \b^* = \min_{j \neq k}  -(\vh^{\top} \x_{j} + \b^*)
\end{equation}
which implies that,
\begin{equation}
    \b^* = \frac{1}{2} \min_{j \neq k}  -\vh^{\top} \x_{j} =  -\frac{1}{2} \max_{j \neq k}  \vh^{\top} \x_{j}
\end{equation}
Then the min margin $\min_{j} margin(\x_{j}) = \b^* = -\frac{1}{2} \max_{j \neq k}  \vh_k^{\top} \x_{j}$. According to problem \ref{eq:max_min_margin}, to find the optimal $\vh_k^*$, we optimize,
\begin{equation}
    \max_{\vh} -\frac{1}{2} \max_{j \neq k}  \vh^{\top} \x_{j}
\end{equation}
which further implies,
\begin{equation}
    \min_{\vh} \max_{j \neq k}  \langle \vw_{j} - \vw_k, \vh \rangle
\end{equation}
which is problem \ref{eq:fix_w_find_h}.
\end{proof}



\begin{figure} [!ht]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Fix_W.png}
         \caption{For the case of $d = 2$, $K = 4$, suppose there are four weight vectors $\{\vw_1, \vw_2,\vw_3,\vw_4\}$ which are distributed on a unit circle with a configuration as shown in the figure.}
         \label{fig:Fix_W}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/margin.png}
         \caption{For fixed $\W$, optimizing feature vector $\vh_1$ for the this problem is equivalent to find a separating hyperplane $\vh_1^{\top} \x + \b = 0$ with the largest margin. \jc{mark two classes with different marker}} 
         \label{fig:margin}
     \end{subfigure}
        \caption{Illustration of Max-Min Margin problem.}         \label{fig:Margin}
\end{figure}







\begin{lemma} \jz{does this imply that if there is no rattler, $h_i=w_i$ must holds for any $i\in [K]$?}Assume 
\begin{equation}\label{eq:min-max-inner-product}
    \mW^\star = \argmin_{\mW} \max_{k}\max_{k'\neq k} \langle \vw_{k'},\vw_k \rangle,  \quad  \st \quad \|\vw_k\|_2 = 1, \forall k.
\end{equation}
If there are multiple global minimizer, then $\mW^\star$ denotes any one of them.
\cy{Moreover, assume that there is no rattler, i.e., $\max_{k\neq k'} \langle \w_{k'}^\star,\w_k^\star \rangle = \max_{k' \ne k''} \langle \w^\star_{k'}, \w_{k''}^\star \rangle$, for all $k''$.}
Then $\mH^\star = \mW^\star$ is the only global minimizer to the following problem
\[
    \min_{\H}  \max_{k \neq k'} \langle \w^\star_{k'} - \w^\star_{k} , \h_k \rangle 
   \quad \st \quad  \|\vh_{k}\|_2 = 1, \forall k
\]
\end{lemma}
\begin{proof} 
Since the problem is separable in terms of $\vh_k$, without loss of generality, we will consider $\vh_1$ as an example. 
Recall that $\mW^\star$ is a global minimizer to $
\min_{\mW} \max_{k}\max_{k'\neq k} \langle \vw_{k'},\vw_k \rangle$. By fixing  $\vw_2^\star,\ldots,\vw_K^\star$, we may conclude that $\vw^\star_1$ is a minimizer to $\min_{\vw_1}\max_{k'\neq 1} \langle \vw^\star_{k'},\vw_1 \rangle$,\zz{rigorous proof? or not correct?} and thus
\[
\max_{k'\neq 1} \langle \vw^\star_{k'},\vw^\star_1 \rangle \le \max_{k'\neq 1} \langle \vw^\star_{k'},\vh \rangle, \ \forall \ \vh\in\mathbb{S}^{d-1},
\]
%\zz{The above requires $\max_{k'\neq 1} \langle \vw^\star_{k'},\vw^\star_1 \rangle = \cdots = \max_{k'\neq K} \langle \vw^\star_{k'},\vw^\star_K \rangle$, is it true?} \zz{This maybe not correct according to \url{http://cohn.mit.edu/spherical-codes}.}
which further implies that 
\[
\max_{k'\neq 1} \langle \vw^\star_{k'} - \vw^\star_1,\vh \rangle \ge \max_{k'\neq 1} \langle \vw^\star_{k'},\vw^\star_1 \rangle - \langle \vw_k^\star, \vh\rangle \ge \langle \vw^\star_{k'},\vw^\star_1 \rangle -1, \ \forall \ \vh\in\mathbb{S}^{d-1},
\]
where the first inequality becomes equality when $\vh = \vw_1^\star$, and the last inequality achieves equality only when $\vh = \vw_1^\star$.
\end{proof}

\begin{proof}[Alternative proof?]
    For any $k$, let
    \begin{equation}
    \begin{split}
        \vh_k^\star &\doteq \arg\min_{\vh_k} \max_{k' \ne k} \langle \w^\star_{k'} - \w^\star_{k} , \h_k \rangle, \quad \st \quad  \|\vh_{k}\|_2 = 1\\
        &= \arg\min_{\vh_k} \Big(- \langle \w^\star_{k} , \h_k \rangle +  \max_{k' \ne k} \langle \w^\star_{k'}, \h_k \rangle \Big), \quad \st \quad  \|\vh_{k}\|_2 = 1.
    \end{split}
    \end{equation}
    By this definition, we have
    \begin{equation}
        - \langle \w^\star_{k} , \h_k^\star \rangle +  \max_{k' \ne k} \langle \w^\star_{k'}, \h_k^\star \rangle \le - \langle \w^\star_{k} , \w^\star_{k} \rangle +  \max_{k' \ne k} \langle \w^\star_{k'}, \w_k^\star \rangle.
    \end{equation}
    Assume for the purpose of arriving at a contradiction that there exist a $\bar{k}$ such that $\vh^\star_{\bar{k}} \ne \vw_{\bar{k}}^\star$. 
    Then it follows that $\langle \vw_{\bar{k}}^\star, \vh_{\bar{k}}^\star \rangle < \langle \vw_{\bar{k}}^\star, \vw_{\bar{k}}^\star \rangle$. 
    Combining this with the inequality above gives
    \begin{equation}\label{eq:prf-max-wh-lt-max-ww}
        \max_{k' \ne \bar{k}} \langle \w^\star_{k'}, \h_{\bar{k}}^\star \rangle < \max_{k' \ne \bar{k}} \langle \w^\star_{k'}, \w_{\bar{k}}^\star \rangle.
    \end{equation}
    Consider $\U \doteq [\u_1, \ldots, \u_K]$, where $\u_{\bar{k}} \doteq \h_{\bar{k}}^\star$ and $\u_k \doteq \w_{k}^\star$ for all $k \ne \bar{k}$. 
    % We claim that 
    % \begin{equation}
    %     \max_{k\neq k'} \langle \u_{k'},\u_k \rangle <  \max_{k\neq k'} \langle \vw_{k'}^\star,\vw_k^\star \rangle,
    % \end{equation}
    % which leads to a contradiction to the optimality of $\mW^\star$. 
    % To establish the theorem we only need to prove that the claim above holds true. 
    Denote
    \begin{multline}
        S \doteq \{(k, k'): k \ne k'\}, \quad 
        S_{\bar{k}}^0 \doteq \{(k, k'): k \ne k', k' \ne \bar{k}, k \ne \bar{k}\}, \\ 
        S_{\bar{k}}^1 \doteq \{(k, k'): k \ne k', k' = \bar{k}\}, \quad 
        S_{\bar{k}}^2 \doteq \{(k, k'): k \ne k', k = \bar{k}\}. 
    \end{multline}
    Note that $S = S_{\bar{k}}^0 \cup S_{\bar{k}}^1 \cup S_{\bar{k}}^2$. Hence,
    \begin{equation}\label{eq:prf-max-uu-le-max-ww}
    \begin{split}
        \max_{k\neq k'} \langle \u_{k'},\u_k \rangle 
        &= \max\{ \max_{S_{\bar{k}}^0} \langle \u_{k'},\u_k \rangle, \max_{S_{\bar{k}}^1} \langle \u_{k'},\u_k \rangle, \max_{S_{\bar{k}}^2} \langle \u_{k'},\u_k \rangle \}\\
        &= \max\{ \max_{S_{\bar{k}}^0} \langle \w_{k'}^\star,\w_k^\star \rangle, \max_{S_{\bar{k}}^1} \langle \h_{\bar{k}}^\star,\w_k^\star \rangle, \max_{S_{\bar{k}}^2} \langle \w_{k'}^\star,\h_{\bar{k}}^\star \rangle \}\\
        &\le \max\{ \max_{S_{\bar{k}}^0} \langle \w_{k'}^\star,\w_k^\star \rangle, \max_{S_{\bar{k}}^1} \langle \w_{\bar{k}}^\star,\w_k^\star \rangle, \max_{S_{\bar{k}}^2} \langle \w_{k'}^\star,\w_{\bar{k}}^\star \rangle \}= \max_{k\neq k'} \langle \w_{k'}^\star,\w_k^\star \rangle,
    \end{split}
    \end{equation}
    where the second equality follows from the definition of $\U$, and the inequality follows from \eqref{eq:prf-max-wh-lt-max-ww}.
    We consider two cases on the inequality in \eqref{eq:prf-max-uu-le-max-ww}.
    \begin{itemize}
        \item The inequality in \eqref{eq:prf-max-uu-le-max-ww} holds as a strict inequality. This leads to a contradiction on the optimality of $\mW^\star$. 
        \item The inequality in \eqref{eq:prf-max-uu-le-max-ww} holds as an equality, i.e., 
            \begin{equation}
                \max_{k\neq k'} \langle \u_{k'},\u_k \rangle = \max_{k\neq k'} \langle \w_{k'}^\star,\w_k^\star \rangle.
            \end{equation}
            In this case, both $\U$ and $\mW^\star$ are optimal solutions to \eqref{eq:min-max-inner-product}, and by our assumption they don't have rattlers. This implies
            \begin{equation}
                \max_{k\neq k'} \langle \u_{k'},\u_k \rangle = \max_{k' \ne \bar{k}} \langle \u_{k'}, \u_{\bar{k}} \rangle, ~~\max_{k\neq k'} \langle \w_{k'}^\star,\w_k^\star \rangle = \max_{k' \ne \bar{k}} \langle \w^\star_{k'}, \w_{\bar{k}}^\star \rangle.
            \end{equation}       
            Combining the three equations above we have
            \begin{equation}
                \max_{k' \ne \bar{k}} \langle \u_{k'}, \u_{\bar{k}} \rangle = \max_{k' \ne \bar{k}} \langle \w^\star_{k'}, \w_{\bar{k}}^\star \rangle.
            \end{equation}
            On the other hand, by combining \eqref{eq:prf-max-wh-lt-max-ww} and the definition of $\U$, we have
            \begin{equation}
                \max_{k' \ne \bar{k}} \langle \u_{k'}, \u_{\bar{k}} \rangle < \max_{k' \ne \bar{k}} \langle \w^\star_{k'}, \w_{\bar{k}}^\star \rangle,
            \end{equation}
            which leads to a contradiction.
    \end{itemize}
\end{proof}


\begin{theorem} If $K \le d+1$, then any global minimimizer $(\mW^\star,\mH^\star)$ of \eqref{eq:min-max-one-sample} must satisfy that $(i)$  $\mW^\star$ forms a simplex ETF, and $(ii)$ $
\mW^\star = \mH^\star.$
\label{thm:K-small-case}\end{theorem}
\begin{proof}
We first consider optimal configuration of $K$ unit-length vectors $\u_1,\ldots,\u_K$. Note that
\begin{align}
& 0 \le \norm{\sum_{k=1}^K \u_k}{2}^2 = \sum_k \sum_{k'} \langle \u_k, \u_{k'} \rangle \le K + K(K-1) \max_{k\neq k'} \langle \u_k, \u_{k'} \rangle,
\end{align}
where the first inequality  achieves equality only when $\sum_{k=1}^K \u_k = 0$ and the second inequality becomes equality only when $\langle \u_k, \u_{k'} \rangle = -\frac{1}{K-1}$ for any $k\neq k'$. These two conditions mean that $\u_1,\ldots,\u_K$ form a simplex ETF. The above equation further impleis that 
\begin{align}
\max_{k\neq k'} \langle \u_k, \u_{k'} \rangle \ge -\frac{1}{K-1}, \ \forall \u_1,\ldots,\u_K \in \mathbb{S}^{d-1},
\label{eq:ETF-requirement}\end{align}
and the equality holds only when $\u_1,\ldots,\u_K$ form a simplex ETF.

We will also need the following result:
\begin{align}
\frac{1}{2}\sum_{k\neq k'}\|\vw_k - \vw_{k'}\|^2 = K^2  - \big\|\sum_{k} \u_k\big\|^2 \le K^2,
\label{eq:proof-ETF-sum}\end{align}
where the last inequality becomes equality when $\sum_{k} \u_k = 0$.

We now use these results to prove \Cref{thm:K-small-case}. Frist note that
\begin{align*}
& K(K-1) \max_{k \neq k'} \langle \w_{k'} - \w_{k} , \h_k \rangle \ge \sum_{k\neq k'} \langle \w_{k'} - \w_{k} , \h_k \rangle = \frac{1}{2} \sum_{k\neq k'} \langle \w_{k'} - \w_{k} , \h_k - \h_{k'} \rangle \\ 
& \ge  -\frac{1}{4} \sum_{k\neq k'}\|\vw_k - \vw_{k'}\|^2 - \frac{1}{4} \sum_{k\neq k'}\|\vh_k - \vh_{k'}\|^2 \ge - K^2,
\end{align*}
where the first inequality achieves equality only when $\langle \w_{k'} - \w_{k} , \h_k \rangle = \langle \w_{j'} - \w_{j} , \h_j\rangle$ for any $k'\neq k, j'\neq j$, the second inequality follows from the Cauchy–Schwarz inequality and acheives inequality only when $\vw_{k'} - \vw_k = \vh_{k'} - \vh_k$ for any $k'\neq k$, and the third inequality follows from \eqref{eq:proof-ETF-sum} and achieves equality only when $\sum_k \vw_k = \sum_k \vh_k = 0$. Assuming all these conditions hold, then  $
 \langle \w_{k'} - \w_{k} , \h_k \rangle = - \frac{K}{K-1}$, which together with the requirement $\vw_{k'} - \vw_k = \vh_{k'} - \vh_k$ implies that
\[
\langle \h_{k'} - \h_{k} , \h_k \rangle = - \frac{K}{K-1}, \quad  \Rightarrow \quad \langle \h_{k'} , \h_k \rangle = - \frac{1}{K-1}, \forall k\neq k',
\]
which holds only when $\mH$ forms a simplex ETF according to the derivation for \eqref{eq:ETF-requirement}. Using the condition  $\vw_{k'} - \vw_k = \vh_{k'} - \vh_k$ which indicates $\langle \w_{k'} , \w_k \rangle = \langle \h_{k'} , \h_k \rangle$, we can obtain that $\mW$ is also a simplex ETF. Moreover, for any $k$, $ -K = \sum_{k'\neq k} \langle \w_{k'} - \w_{k} , \h_k \rangle = -K \langle\w_{k} , \h_k\rangle$ (since $\sum_k \w_k = 0$), we conclude $\vw_k = \vh_k$.

\end{proof}

\zz{Some useful observation:
\[
\sum_{k,k'\in[K]} (\vw_{k'} - \vw_k)^\top \vh_k = \frac{1}{2}\sum_{k,k'\in[K]} (\vw_{k'} - \vw_k)^\top (\vh_k - \vh_{k'})
\]
}


\begin{theorem} If $K \ge d+2$, then 
\[
\max_{k\neq k'} \langle \u_k, \u_{k'} \rangle \ge 0
\]
always holds. 
The inequality achieves equality when $K \le 2d$ and choose $\u_1,\ldots,\u_K$ from the vertices of the cross-polytope $\{\pm \e_1, \ldots,\pm \e_d\}$ where $\{\e_1, \ldots,\e_d\}$ form an orthonormal matrix. \zz{This is  sufficient but not necessary for achiving equality, e.g., $K = 5, d =3$ has different solutions with minimal angle 90 degree.  CE loss always finds solution with minimal angle 90 degree when $d+2\le K \le 2d$. Could we prove this?}
\end{theorem}
\begin{proof}
\zz{Any simple proof?}
\end{proof}







\newpage
Then the loss is,
\begin{equation}
\begin{aligned}
    f(\W,\H) &=  \frac{1}{nK} \sum_{k = 1}^{K} \sum_{i= 1}^{n} \log(\sum_{k^{'} =1}^{K} \exp(\tau \langle \w_{k^{'}} - \w_k, \h_{k,i} \rangle) \\
    &= \frac{1}{nK} \sum_{k = 1}^{K} \sum_{i= 1}^{n} \log(1+ \sum_{k^{'} \neq k}^{K} \exp(\tau \langle \w_{k^{'}} - \w_k, \h_{k,i} \rangle) \\
    & \approx \frac{1}{nK} \sum_{k = 1}^{K} \sum_{i= 1}^{n} \log(\sum_{k^{'} \neq k}^{K} \exp(\tau \langle \w_{k^{'}} - \w_k, \h_{k,i} \rangle)
\end{aligned}
\end{equation}
The $LogSumExp(LSE)$ function's domain is $\mathbb{R}^K$, $LSE(x) = \log(\sum_{i = 1}^{K} \exp(x_i))$, and it is an approximation to $\max$ function with the following bounds,
\begin{equation}
    \max \{x_1, x_2, \cdots, \x_K\} \leq LSE(x) \leq \max \{x_1, x_2, \cdots, \x_K\} + \log(K)
\end{equation}
For our CE loss, 
\begin{equation}
    \frac{1}{nK} \sum_{k = 1}^{K} \sum_{i= 1}^{n} \max_{k^{'} \neq k} \tau \langle \w_{k^{'}} - \w_k, \h_{k,i} \rangle \leq f(\W,\H) \leq \frac{1}{nK} \sum_{k = 1}^{K} \sum_{i= 1}^{n} \max_{k^{'} \neq k} \tau \langle \w_{k^{'}} - \w_k, \h_{k,i} \rangle + \log(K-1)
\end{equation}
Dividing by $\tau$ gives,
\begin{equation}
    \frac{1}{nK} \sum_{k = 1}^{K} \sum_{i= 1}^{n} \max_{k^{'} \neq k} \langle \w_{k^{'}} - \w_k, \h_{k,i} \rangle \leq \frac{1}{\tau}f(\W,\H) \leq \frac{1}{nK} \sum_{k = 1}^{K} \sum_{i= 1}^{n} \max_{k^{'} \neq k} \langle \w_{k^{'}} - \w_k, \h_{k,i} \rangle + \frac{\log(K-1)}{\tau}
\end{equation}
So if $\tau \rightarrow \infty$, then $\log(K-1) / \tau \rightarrow 0$. It means that the $LSE$ function would converge to a trivial distribution with all mass concentrated on the highest-probability class which is $max$ function. Then the optimization problem would converge to,
\begin{equation} 
\begin{aligned}
    \min_{\W,\H} \quad & f(\W,\H) := \frac{1}{nK} \sum_{k = 1}^{K} \sum_{i= 1}^{n} \max_{k^{'} \neq k}\tau \langle \w_{k^{'}} - \w_k, \h_{k,i} \rangle  \\
    \st \quad & \|\vw_k\|_2 = 1, \ \|\vh_{k,i}\|_2 = 1.
\end{aligned}
\end{equation}
 We will study one sample per class since the problem on features can be decoupled, then
\begin{equation} \label{eq:maxinnerproduct}
\begin{aligned}
    \argmin_{\|\vw_k\|_2 = 1, \ \|\vh_{k}\|_2 = 1} \sum_{k = 1}^{K} \max_{k^{'} \neq k}\langle \w_{k^{'}} - \w_k, \h_{k} \rangle
\end{aligned}
\end{equation}



\begin{theorem}\label{thm:d=2global}
Consider classifier weight vector and feature vector on unit sphere $\{ \w_k \in \mathbb{S}^{d-1}\}_{k = 1}^{K}$ and $\{ \h_{i} \in \mathbb{S}^{d-1}\}_{i = 1}^{nK}$. If $d = 2$, the global minimum of problem \ref{eq:maxinnerproduct} is the uniform distribution on circle with,
\begin{equation}
    \w_k^* = \h_{k}^* = \left[\cos(\frac{2\pi}{K}k),\sin(\frac{2\pi}{K}k)\right]^{\top}
\end{equation}
\end{theorem}

\begin{proof}
    [Proof of Theorem \ref{thm:d=2global}]
    
    
\end{proof}

\begin{theorem}\label{thm:uniform}
Consider classifier with weight vectors on unit spheres $\{ \w_k \in \mathbb{S}^{d-1}\}_{k=1}^{K}$, If $d = 2$, then optimizing
 \begin{equation}
     \w_k^* = \argmin_{\|\w_k\|_2 = 1} \quad \sum_{k = 1}^{K} (\max_{k^{'} \neq k} \langle \w_{k^{'}}, \w_{k}\rangle)
 \end{equation}
would lead to the uniform distribution on unit sphere. Suppose $\w_k =[\cos(\alpha_k), \sin(\alpha_k)]^{\top}$, and $ 0 = \alpha_1 \leq \alpha_2 \cdots \leq \alpha_k \leq 2\pi$, then the optimal solution is $\alpha_k = \frac{2\pi}{K}k$.

\end{theorem}

\begin{proof} 

[Proof of Theorem \ref{thm:uniform}]
For weight vectors on unit spheres, If $d = 2$, $\w_k =[cos(\alpha_k), sin(\alpha_k)]^{\top}$, since maximizing the pair-wise inner product is equivalent to minimizing the pair-wise angle, then the problem can be rewritten as,

\begin{equation}
    \argmax_{0 = \alpha_1 \leq \alpha_2 \cdots \leq \alpha_k \leq 2\pi} \quad \sum_{k = 1}^{K}(\min_{k^{'} \neq k}(|\alpha_{k^{'}} - \alpha_k|))
\end{equation}
Define the pair-wise angle absolute value as $\theta_k = |\alpha_{k+1} - \alpha_{k}|$ for $ \k = \{1, \cdots, K-1 \}$ and $\theta_K = |\alpha_K - 2\pi|$, so $\theta_i \geq 0 $ , then for $k = 1$, 
\begin{equation}
    \min_{\theta_1, \cdots, \theta_K} \quad \{\theta_1, (\theta_2+\theta_1), \cdots, (\theta_{K-1}+\cdots+ \theta_{1}) + \theta_{K}\} = \min_{\theta_1, \cdots, \theta_K} \{ \theta_1, \theta_{K}\} 
\end{equation}
Similarly simplification for $k = 2 , \cdots , K$, then optimization problem is,
\begin{equation}
\begin{aligned}
    \argmax_{\theta_1, \theta_2, \cdots, \theta_{K}} \quad & \sum_{k = 1}^{K-1} (\min \{\theta_{k+1}, \theta_{k}\}) + \min \{\theta_{1}, \theta_{K}\} \\
    \textrm{s.t.} \quad & \theta_1 + \cdots + \theta_K = 2\pi\\
    & 0 \leq \theta_k \leq 2\pi \\
\end{aligned}
\end{equation}
The $\min(x,y) = \frac{1}{2}(x+y - |x-y|)$ a then
\begin{equation}
\begin{aligned}
   \argmax_{\theta_1, \theta_2, \cdots, \theta_{K}} \quad &  4\pi - (\sum_{k =1}^{K-1} (|\theta_k - \theta_{k+1}|) + |\theta_K - \theta_1|) \\
   \textrm{s.t.} \quad & \theta_1 + \cdots + \theta_K = 2\pi\\
\end{aligned}
\end{equation}
And $\theta_K = 2\pi - (\theta_1 + \cdots + \theta_{K-1})$, 
\begin{equation}
   \argmin_{\theta_1, \theta_2, \cdots, \theta_{K-1}} \quad \sum_{k =1}^{K-1}(|\theta_k - \theta_{k+1}| )+ |2\pi - (\theta_1 + \cdots + \theta_{K-1}) - \theta_1|
\end{equation}
For each term the minimum value of absolute function is zero, so the solution is $\theta_1 = \theta_2 = \cdots =\theta_K = \frac{2 \pi}{K}$, and the optimal solution is $\alpha_k = \frac{2\pi}{K}k$.

\end{proof} 

\begin{theorem}\label{thm:alignment}
Consider feature vectors on unit sphere $\{ \h_k \in \mathbb{S}^{d-1}\}_{k=1}^{K}$, If $d = 2$, and we fix classifier weight vector $\w_k$ as the uniform distribution which is the solution of \ref{thm:uniform}, then optimizing
\begin{equation}
    \argmin_{\|\h_k\|_2 =1} \quad \sum_{k= 1}^{K} \max_{k^{'} \neq k} \langle \w_{k^{'}}^* - \w_{k}^* , \h_k \rangle
\end{equation}
would lead to alignment between feature and classifier weight as $\h_k = \w_k^*$.

\end{theorem}

\begin{proof} 

[Proof of Theorem \ref{thm:alignment}]

Firstly consider the case of $k = 1$ and the optimization problem is
\begin{equation}
    \argmin_{\|\h\|_2 =1} \quad \max_{k^{'} \neq 1} \langle \w_{k^{'}}^* - \w_{1}^* , \h \rangle
\end{equation}
Define the feature vector as $\h = [cos(\alpha), sin(\alpha)]$, uniform distributed weight as $\w_k^* = \left[\cos(\frac{2\pi}{K}(k-1)), \sin(\frac{2\pi}{K}(k-1))\right]^{\top}$, $\w_1^* = [1,0]^{\top}$. So the optimization problem can be rewritten as
\begin{equation}
\begin{aligned}
    \argmin_{\alpha} \quad & \max_{k^{'} \neq 1} ( \cos(\frac{2\pi}{K}(k^{'}-1) - \alpha) -\cos(\alpha)) \\
    \argmin_{\alpha} \quad & \max_{k \neq 0} (\cos(\frac{2\pi}{K}k - \alpha) -\cos(\alpha) )\\
    \argmin_{\alpha} \quad & \max_{k \neq 0} (-2\sin(\frac{\pi}{K}k) \sin(\frac{\pi}{K}k - \alpha))
\end{aligned}
\end{equation}
Define the absolute angle between $\w_k^* - \w_1^* $ and $\h$ is $\theta_k$, if $\frac{\pi}{K} \leq \alpha \leq \pi$ or $ -\pi \leq \alpha \leq -\frac{\pi}{K}$, then there exists a $\w_k^*$ whose $\theta_k$ is small than 90 degree which means that this term $\max_{k^{'} \neq 1} \langle \w_{k^{'}}^* - \w_{1}^* , \h \rangle$ would be positive. If $-\frac{\pi}{K} \leq \alpha \leq \frac{\pi}{K}$, all $\theta_k$ would large than 90 degree and this term would be negative. As we're looking for the $\argmin$ of the $\max$ function, we will only consider the situation $-\frac{\pi}{K} \leq \alpha \leq \frac{\pi}{K}$. Then, 
\begin{equation}
\begin{aligned}
    \argmin_{\alpha} \quad & \max_{k \neq 0} (-2\sin(\frac{\pi}{K}k) \sin(\frac{\pi}{K}k - \alpha)) \\
    \textrm{s.t.} \quad & -\frac{\pi}{K} \leq \alpha \leq \frac{\pi}{K}\\
\end{aligned}
\end{equation}
We have $\langle \w_{k}^* - \w_{1}^* , \h \rangle = \|\w_{k^{'}}^* - \w_{1}^*\| \cos(\theta_k)$, to find the maximum of this term, we need to find a $\w_k$ with smaller $\theta_k$ and smaller vector length $\|\w_{k}^* - \w_{1}^*\|$. Since $\theta_1$ and $\theta_{K-1}$ satisfy both of them, then the problem is
\begin{equation}
\begin{aligned}
    \argmin_{\alpha} \quad & \max_{\{k = 1, k = K-1\} }(-2\sin(\frac{\pi}{K}k) \sin(\frac{\pi}{K}k - \alpha)) \\
    \textrm{s.t.} \quad & -\frac{\pi}{K} \leq \alpha \leq \frac{\pi}{K}\\
\end{aligned}
\end{equation}

For $0 \leq \alpha \leq \frac{\pi}{K}$, $\theta_1$ is smaller than $\theta_{K-1}$, so the problem becomes,
\begin{equation}
\begin{aligned}
    \argmin_{\alpha} \quad & -2\sin(\frac{\pi}{K}k) \sin(\frac{\pi}{K}k - \alpha) \\
    \textrm{s.t.} \quad & 0 \leq \alpha \leq \frac{\pi}{K}\\
\end{aligned}
\end{equation}
The function is monotonically increasing under this constraint so the solution is $\alpha = 0$. 

For $-\frac{\pi}{K} \leq \alpha \leq 0$, $\theta_{K-1}$ is smaller than $\theta_{1}$, so the problem becomes,
\begin{equation}
\begin{aligned}
    \argmin_{\alpha} \quad & -2\sin(\frac{\pi}{K}(k-1)) \sin(\frac{\pi}{K}(k-1) - \alpha) \\
    \textrm{s.t.} \quad & -\frac{\pi}{K} \leq \alpha \leq 0\\
\end{aligned}
\end{equation}
The function is monotonically decreasing under this constraint so the solution is $\alpha = 0$. 

In conclusion, the optimal solution is $\h^* = \left[\cos(\alpha), sin(\alpha)\right]^{\top} = [1,0]^{\top} = w_1^*$. Similarly, we can get $h_k^* = w_k^*$ for all other cases. 
\end{proof}

\zz{@Jiachen, could we then combine the above results together to show the global solution for \eqref{eq:min-max-prob} when $d = 2$?}




\paragraph{Assumption of ${\mc L}$ for Within-class collapsing:} Assume ${\mc L}(\z,\y_k)$ is convex in $\z$. Then for any fixed $\W$, $f(\W,\H)$ can be  decoupled into a sum of sub-functions in terms of $\h_{k,i}$ and each sub-function is strongly convex. Thus, for each $k=1, \ldots, K$ we have $\h_{k,i}^* \equiv \h_{k}^*, \forall i$. 

Based on the above result, it is sufficient to analyze the case where each class has one sample. To avoid the scaling issue, we first consider the case of optimizing the features and classifiers on the sphere. Gradient and Hessian of $\cL$ are given by
\begin{align*}
& \cL(\z,\y_k) = - \log(\e_k^\top \sigma(\z))\\
& \nabla_{\z}\cL(\z,\y_k) = \sigma(\z) -\e_k, \ \text{where $\sigma$ is the soft-max function},\\
& \nabla^2_{\z}\cL(\z,\y_k) = \diag(\sigma(\z)) - \sigma(\z)\sigma(\z)^\top
\end{align*}

Denote by $\mZ = \W^{\top}\H$ and $g(\mZ)=f(\W,\H)$. Let $\g^i$ and $\g_k$ denote the $i$-th row and $k$-th column of $\nabla g(\mZ)$, respectively. Recall that $\nabla g(\mZ) = \begin{bmatrix}\sigma(\z_1) - \e_1 & \cdots & \sigma(\z_K) - \e_K \end{bmatrix}$. Then the Riemannian gradient and Hessian are given by
\begin{align*}
& \grad_{\w_k} = \nabla_{\w_k} f(\W,\H) - \w_k \w_k^\top \nabla_{\w_k} f(\W,\H) = \mH \g^k - \w_k \underbrace{\w_k^\top \mH \g^k}_{\alpha_k},\\
& \grad_{\h_k} = \nabla_{\h_k} f(\W,\H) - \h_k \h_k^\top \nabla_{\h_k} f(\W,\H) = \W \g_k - \h_k \underbrace{\h_k^\top \W \g_k}_{\beta_k}.
\end{align*}

The oblique manifold $\cM = \mathcal{OB}(p,q)$ is a product of $q$ unit spheres $\mathbb{S}^{p-1}$
\begin{equation}
\cM = \mathcal{OB}(p,q) = \{\mZ \in \RR ^{p \times q} | \diag(\mZ ^{\top} \mZ) = 1\}
\end{equation}
Correspondingly, the tangent space $T_{\X} \mathcal{OB}(p,q)$ is
\begin{equation}
    T_{\X} \mathcal{OB}(p,q) = \{\mZ \in \RR ^{p \times q} | \diag(\X ^{\top} \mZ) = 0 \}
\end{equation}
and the projection operator $\mathcal{P}_{T_{\X} \mathcal{OB}(p,q)}$ is 
\begin{equation}
    \mathcal{P}_{T_{\X} \mathcal{OB}(p,q)}(\mZ) = [(\I - \x_{1} \x_{1}^{\top}) \z_{1}, \ldots, (\I - \x_{q} \x_{q}^{\top}) \z_{q}]
\end{equation}


The Riemannian Hessian bilinear form of $f(\W,\H)$ along any direction $\\Delta = (\\Delta_{\W}, \\Delta_{\H}) \in T_{\W} \mathcal{OB}(d,K) \times T_{\H} \mathcal{OB}(d,K)$ by
\begin{equation}
    \Hess f(\W,\H)[\\Delta, \\Delta] = \nabla^2f(\W,\H)[\\Delta,\\Delta] - \langle \\Delta_{\W} \ddiag(\mZ \nabla g(\mZ)^T),\\Delta_{\W} \rangle - \langle \\Delta_{\H} \ddiag(\mZ^T \nabla g(\mZ) ),\\Delta_{\H}\rangle
\end{equation}
Where, for any $\\Delta \in \RR^{d \times K} \times \RR^{d \times K}$, the Hessian bilinear form of $f(\W, \H)$ along the direction $\\Delta$ by
\begin{equation} \label{eq:Riemannian_Hessian}
    \nabla^2f(\W,\H)[\\Delta,\\Delta] = \nabla^2 g(\mZ)[\W^T \\Delta_{\H} + \\Delta_{\W}^T\H , \W^T \\Delta_{\H} + \\Delta_{\W}^T\H ] + 2 \langle  \nabla g(\mZ), \\Delta^{T}_{\W}\\Delta_{\H} \rangle 
\end{equation}


We denote the set of all Riemannian critical points by 
\begin{equation}
    \mathcal{C} := \{ (\W,\H) \in \mathcal{OB}(d,K) \times \mathcal{OB}(d,K) | \grad_{\W} f(\W, \H) = 0, \grad_{\H}f(\W, \H) = 0 \}
\end{equation}
Riemannian critical points satisfy first-order optimality condition
\begin{equation}\label{eq:Critial_Cond}
\begin{aligned}
    \H \G^T &= \W \diag(\boldsymbol{\alpha})  \\
    \W \G &= \H \diag(\boldsymbol{\beta})
\end{aligned}
\end{equation}

where $\boldsymbol{\alpha} = [\alpha_{1}, \cdots, \alpha_{K}]$, $\boldsymbol{\beta} = [\beta_{1}, \cdots, \beta_{K}]$, $\alpha_{k} = \w_{k}^T \H \g^{k}$, $\beta_{k} = \h_{k}^T \W \g_{k}$.


Any low dimensional critical points in $\RR^{d}$ are also critical points in high dimension space of $\RR^{d+1}$. Suppose $\W \in \RR^{d \times K}$, $\H \in \RR^{d \times K}$ are critical points in $\RR^{d}$,
$\widetilde{\W} = \left[\begin{array}{ c }
    \W  \\
    \hline
    \boldsymbol{0}
\end{array}\right] \in \RR^{(d+1) \times K}$, $\widetilde{\H} = \left[\begin{array}{ c }
\H \\
\hline
\boldsymbol{0}
\end{array}\right] \in \RR^{(d+1) \times K}$, 
\begin{equation}
    \widetilde{\mZ} = \widetilde{\W}^T \widetilde{\H} = [\W^T |  \boldsymbol{0}^T] \left[\begin{array}{ c }
\H \\
\hline
\boldsymbol{0}
\end{array}\right] = \W^T\H = \mZ
\end{equation}
Then $\widetilde{\G} = \G$, $\widetilde{\beta}_{k} = \beta_{k}$, 
\begin{equation}
    \widetilde{\W}\widetilde{\G} = \left[\begin{array}{ c }
    \W  \\
    \hline
    \boldsymbol{0}
\end{array}\right] \G = \left[\begin{array}{ c }
    \W \G  \\
    \hline
    \boldsymbol{0}
\end{array}\right] = \left[\begin{array}{ c }
    \H \diag(\boldsymbol{\beta})  \\
    \hline
    \boldsymbol{0}
\end{array}\right] = \widetilde{\H}\diag( \widetilde{\boldsymbol{\beta}})
\end{equation}
Similarly, $\widetilde{\H} \widetilde{\G}^T = \widetilde{\W} \diag(\widetilde{\boldsymbol{\alpha}})$. So $\widetilde{\H}$ and $\widetilde{\W}$ also satisfy first-order optimality condition which are Riemannian critical points in $\RR^{d+1}$.


Assume there exists a critical point $(\W, \H) \in \mathcal{C}$ which satisfies $\h_{k} = \w_{k}$ for $k = 2, \ldots,K$ but $\h_{1} \neq \w_{1}$. We want to prove that this critical point is not a local minimum. So we need to find a direction $\\Delta = (\\Delta_{\W}, \\Delta_{\H}) \in T_{\W} \mathcal{OB}(d,K) \times T_{\H} \mathcal{OB}(d,K)$ along which the Riemannian Hessian has a strictly negative curvature at this point.
\begin{equation}
    \Hess f(\W, \H)[\\Delta, \\Delta] < 0
\end{equation}
We choose a direction which pushes $\h_{1}$ and $\w_{1}$ closer
\begin{equation}
\begin{aligned}
    \boldsymbol{\Delta}_{\W} &= \mathcal{P}_{T_{\W}\mathcal{OB}(d,K)}([\h_{1}, 0,0,\ldots,0])  = [(\I - \w_{1}\w_{1}^T)\h_{1}, 0,0,\ldots,0] = [\boldsymbol{\delta}_{\W}, 0,0,\ldots,0]\\
    \boldsymbol{\Delta}_{\H} &= \mathcal{P}_{T_{\H}\mathcal{OB}(d,K)}([\w_{1}, 0,0,\ldots,0]) = [(\I - \h_{1}\h_{1}^T)\w_{1}, 0,0,\ldots,0] = [\boldsymbol{\delta}_{\H}, 0,0,\ldots,0]\\
\end{aligned}
\end{equation}
According to \eqref{eq:Critial_Cond}
\begin{equation} \label{eq:term1}
\begin{aligned}
\langle \boldsymbol{\Delta}_{\W} \ddiag(\mZ \nabla g(\mZ)^T),\boldsymbol{\Delta}_{\W} \rangle &= \langle \boldsymbol{\Delta}_{\W} \ddiag(\W^T\W \diag(\boldsymbol{\alpha})),\boldsymbol{\Delta}_{\W} \rangle \\
&= \langle [\alpha_{1} \boldsymbol{\delta}_{\W}, 0 \cdots, 0],[\boldsymbol{\delta}_{\W}, \cdots, 0] \rangle = \alpha_{1} \|\boldsymbol{\delta}_{\W}\|^2 
\end{aligned}
\end{equation}

\begin{equation}\label{eq:term2}
\begin{aligned}
\langle \boldsymbol{\Delta}_{\H} \ddiag(\mZ^T \nabla g(\mZ)),\boldsymbol{\Delta}_{\H} \rangle &= \langle \boldsymbol{\Delta}_{\H} \ddiag(\H^T\H\diag(\boldsymbol{\beta})),\boldsymbol{\Delta}_{\H} \rangle \\
&= \langle [\beta_{1} \boldsymbol{\delta}_{\H}, 0 \cdots, 0],[\boldsymbol{\delta}_{\H}, \cdots, 0] \rangle = \beta_{1} \|\boldsymbol{\delta}_{\H}\|^2
\end{aligned}
\end{equation}
According to \eqref{eq:Riemannian_Hessian}, \eqref{eq:term1} and \eqref{eq:term2}, the Riemannian Hessian is
\begin{equation}
    \Hess f(\W,\H)[\boldsymbol{\Delta}, \boldsymbol{\Delta}] = \nabla^2\g(\mZ)[\boldsymbol{\Delta}_{\M}, \boldsymbol{\Delta}_{\M}] 
    + 2  \nabla g(\mZ)_{11} \boldsymbol{\delta}_{\W}^T\boldsymbol{\delta}_{\H} - \alpha_{1}\|\boldsymbol{\delta}_{\W} \|^2 - \beta_{1}\|\boldsymbol{\delta}_{\H} \|^2
\end{equation}

Where $\boldsymbol{\delta}_{\W} = (\I - \w_{1}\w_{1}^T)\h_{1}$, $\boldsymbol{\delta}_{\H} = (\I - \h_{1}\h_{1}^T)\w_{1}$,  $\alpha_{1} = \w_{1}^T \H \g^{1}$, $\beta_{1} = \h_{1}^T \W \g_{1}$, $\nabla g(\mZ)_{11}  = \sigma(\z_{1})[1] - 1$ and 
\begin{equation}
    \begin{aligned}
        \nabla^2\g(\mZ)[\boldsymbol{\Delta}_{\M}, \boldsymbol{\Delta}_{\M}] = \frac{1}{K} \sum_{i=1}^{K} \boldsymbol{\delta}_{\M_{i}}^T[\diag(\sigma(\z_{i})) - \sigma(\z_{i})\sigma(\z_{i})^T]\boldsymbol{\delta}_{\M_{i}}
    \end{aligned}
\end{equation}


Let $\boldsymbol{\delta}_{\M_{i}}$ denote the $i$-th column of $\boldsymbol{{\Delta}}_{\M} = \W^T \boldsymbol{\Delta_{\H}} + \boldsymbol{\Delta_{\W}}^T \H$
\begin{equation}
    \boldsymbol{{\Delta}}_{\M} = 
    \begin{bmatrix}
\| \boldsymbol{\delta}_{\W}\|^2 + \| \boldsymbol{\delta}_{\H}\|^2& \boldsymbol{\delta}_{\W}^T \h_{2} & \cdots & \boldsymbol{\delta}_{\W}^T \h_{K}\\
\boldsymbol{\delta}_{\H}^T \w_{2} & 0 & \cdots & 0\\
\vdots & \vdots & \ddots & \vdots \\
\boldsymbol{\delta}_{\H}^T \w_{K} & 0 & \cdots & 0 \\
\end{bmatrix}
\end{equation}


\begin{conjecture}\label{conj:full-row rank}
    If $\W$ and $\H$ are full row rank, and they satisfy first-order optimality condition \eqref{eq:Critial_Cond}, then $\W = \H$.
\end{conjecture}
If $\W$ and $\H$ are full row rank, $\W\W^T$ and $\H\H^T$ are invertible matrix. 
\begin{equation}
    \W \G \H^T = \H \G^T \W^T = \H \diag(\boldsymbol{\beta}) \H^T = \W \diag(\boldsymbol{\alpha}) \W^T
\end{equation}

\begin{equation}
    \W \W^T \H \H^T - \W\H^T - \H \H^T\W\W^T + \H \W^T = \0
\end{equation}

\end{proof}

New direction 1: The Hessian is complicated if we push $\h_{1}$ and $\w_{1}$ closer to each other at the same time. So we choose a new direction which pushes $\h_{1}$ closer toward $\w_{1}$ while holding $\w_{1}$ unchanged. 
\begin{equation}
\begin{aligned}
    \boldsymbol{\Delta}_{\W} &= [\mathbf{0}, \mathbf{0},\mathbf{0},\ldots,\mathbf{0}]\\
    \boldsymbol{\Delta}_{\H} &= \mathcal{P}_{T_{\H}\mathcal{OB}(d,K)}([\w_{1}, \mathbf{0},\mathbf{0},\ldots,\mathbf{0}]) = [(\I - \h_{1}\h_{1}^T)\w_{1}, \mathbf{0},\mathbf{0},\ldots,\mathbf{0}] = [\boldsymbol{\delta}_{\H}, \mathbf{0},\mathbf{0},\ldots,\mathbf{0}]\\
\end{aligned}
\end{equation}
According to \eqref{eq:Riemannian_Hessian}, \eqref{eq:term1} and \eqref{eq:term2}, the Riemannian Hessian is
\begin{equation}
\begin{aligned}
    \Hess f(\W,\H)[\boldsymbol{\Delta}, \boldsymbol{\Delta}] &= \nabla^2\g(\mZ)[\boldsymbol{\Delta}_{\M}, \boldsymbol{\Delta}_{\M}]  - \beta_{1}\|\boldsymbol{\delta}_{\H} \|^2 \\
    &= \frac{1}{K} \boldsymbol{\delta}_{\M}^T[\diag(\sigma(\z_{1})) - \sigma(\z_{1})\sigma(\z_{1})^T]\boldsymbol{\delta}_{\M} - \beta_{1}\|\boldsymbol{\delta}_{\H} \|^2
\end{aligned}
\end{equation}

Define $\boldsymbol{\delta}_{\M} = [\boldsymbol{w}_1^T \boldsymbol{\delta_H}, \boldsymbol{w}_2^T \boldsymbol{\delta_H}, \cdots, \boldsymbol{w}_K^T \boldsymbol{\delta_H}]^T = [x_1,x_2, \cdots, x_K]$, and $\sigma(\z_{1}) = [ \sigma_{1}, \sigma_{2}, \cdots, \sigma_{K}]$, $\|\boldsymbol{\delta}_{\H} \|^{2} = x_1$. The Riemannian Hessian is 
\begin{equation}
\begin{aligned}
    \Hess f(\W,\H)[\boldsymbol{\Delta}, \boldsymbol{\Delta}] &= \frac{1}{K}(\sum_{k = 1}^{K} \sigma_{k} x_{k}^2 - (\sum_{k = 1}^{K} \sigma_{k} x_{k})^2) - \beta_1 x_1
\end{aligned}
\end{equation}
We can use the critical point condition $ \W \g_1 = \h_1 \beta_1$ and $\beta_1 = \h_1^T \W \g_1$ to simplify $\beta_1 x_1$ ,
\begin{equation}
\begin{aligned}
    \beta_1 x_1 &= \beta_1 \w_1^T (\I - \h_1 \h_1^T)\w_1 \\
    &= \beta_1 - \w_1^T \W \g_1 \h_1^T \w_1 \\
    &= \h_1^T (\I - \w_1\w_1^T) \W \g_1 \\
    &= \sum_{k =2}^{K} \sigma_k \w_k^T (\I - \w_1 \w_1^T)\h_1
    &= \sum_{k =1}^{K} \sigma_k \w_k^T \boldsymbol{\delta}_{\W}
\end{aligned}
\end{equation}

In summary, the Riemannian Hessian at the critical point along designed direction $\boldsymbol{\Delta}$ is,
\begin{equation}
    \begin{aligned}
        \Hess f(\W,\H)[\boldsymbol{\Delta}, \boldsymbol{\Delta}] &= \frac{1}{K} (\sum_{k = 1}^{K} \sigma_k(x_k^2 - K y_k) - (\sum_{ k =1}^K \sigma_k x_k)^2)
    \end{aligned}
\end{equation}
where $x_k = \w_k^T \boldsymbol{\delta}_{\H}$,$y_k = \w_k^T \boldsymbol{\delta}_{\W}$, $\sigma_k = \frac{\exp(\w_k^T \h_1)}{ \sum_{i = 1}^{K} \exp(\w_i^T \h_1)} $, $\boldsymbol{\delta}_{\H} = (\I - \h_1 \h_1^T) \w_1$,$\boldsymbol{\delta}_{\W} = (\I - \w_1 \w_1^T) \h_1$.

New direction 2: If we choose the direction which pushes $\w_1$ closer toward $\h_1$, similarly:
\begin{equation}
\begin{aligned}
    \boldsymbol{\Delta}_{\W} &= \mathcal{P}_{T_{\W}\mathcal{OB}(d,K)}([\h_{1}, \boldsymbol{0},\boldsymbol{0},\ldots,\boldsymbol{0}])  = [(\I - \w_{1}\w_{1}^T)\h_{1}, \boldsymbol{0},\boldsymbol{0},\ldots,\boldsymbol{0}] = [\boldsymbol{\delta}_{\W}, \boldsymbol{0},\boldsymbol{0},\ldots,\boldsymbol{0}]\\
    \boldsymbol{\Delta}_{\H} &= [\boldsymbol{0}, \boldsymbol{0},\boldsymbol{0},\ldots,\boldsymbol{0}]\\
\end{aligned}
\end{equation}
Then the Riemannian Hessian at the critical point along designed direction $\Delta$ is
\begin{equation}
    \Hess f(\W,\H)[\boldsymbol{\Delta}, \boldsymbol{\Delta}] = \frac{1}{K} \sum_{k = 1}^{K} \hat{\sigma}_k(\hat{x}_k^2(1 - \hat{\sigma}_k) - K \hat{y}_k)
\end{equation}

where $\hat{x}_k = \h_k^T \boldsymbol{\delta}_{\W}$,$\hat{y}_k = \h_k^T \boldsymbol{\delta}_{\H}$, $\hat{\sigma}_k = \frac{\exp(\w_1^T \h_k)}{ \sum_{i = 1}^{K} \exp(\w_i^T \h_k)} $, $\boldsymbol{\delta}_{\H} = (\I - \h_1 \h_1^T) \w_1$,$\boldsymbol{\delta}_{\W} = (\I - \w_1 \w_1^T) \h_1$.


\jc{There are three conditions we need to consider:1.first-order optimal condition; 2. $\W,\H$ is not aligned which is $\W \neq \H$. 3.$\W \W^T$ and $\H \H^T$ are full rank. Does it exist for a specific $\W,\H$ which satisfies all 3 conditions? We assume it exists but how can we find an example through algorithm? What if it doesn't exist?}

\begin{theorem}\label{thm:main}
    If conjectures \ref{conj:within-class-collapsing}, \ref{conj:self-duality}, and \ref{conj:equal-norm} hold true, we have
    \begin{itemize}
        \item If $\mc L$ is the MSE loss, then
        \begin{equation}\label{eq:optimal-W-MSE}
            \W^* = \arg\min_{\W} \sum_{k \ne k'} \left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_{k'}}{\|\w_k\|_2} \right\rangle ^2.
        \end{equation}
        That is, the averaged pairwise angle between rows of $\W^*$ is maximized.
        \item If $\mc L$ is the CE loss, we have
        \begin{equation}\label{eq:optimal-W-CE}
            \W^* = \arg\min_{\W} \sum_{k=1}^K \log\left( \exp(1) + \sum_{k' \ne k} \exp \left(\left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2} \right\rangle\right) \right).
        \end{equation}
        Since LogSumExp is an approximation of the maximum function, if we ignore the constant $\exp(1)$\footnote{Or, can we argue that when the maximum is a constant (\ie, $1$), LogSumExp approximates in some sense the second maximum?}, this is saying that approximately the minimum pairwise angle between rows of $\W^*$ is maximized. More precisely, 
        \begin{multline}
            \log 2 + \max_{k' \ne k} \left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2} \right\rangle
            \le
            \log\left( \exp(1) + \sum_{k' \ne k} \exp \left(\left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2} \right\rangle\right) \right)\\
            \le 
            \log (\exp(2)+k-1) + \max_{k' \ne k} \left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2} \right\rangle
        \end{multline}
    \end{itemize}
\end{theorem}



By Theorem~\ref{thm:main}, the objectives of both MSE and CE can be interpreted as encouraging the classifier weights associated with different classes to be \emph{spread out}, and their difference lies in how the notion of ``spread out'' is defined. 
Intuitively, MSE encourages the classes to be separated \emph{on average}, while CE encourages that every pair of classes are separated (similar result exists for contrastive loss \cite{wang2020understanding}). 
Such a difference may explain why MSE loss is often observed to produce inferior performance, with the following argument: With the MSE loss, certain pairs of classes may be very close to each other in the feature space hence less distinguishable (as Zhihui has observed), leading to large classification errors (do we observe this in practice?).

Questions:

\begin{itemize}
    \item When $d > N$, can we prove that the solution to \eqref{eq:optimal-W-MSE} and \eqref{eq:optimal-W-CE} is simplex ETF?
    \item When $d < N$, can we prove that the solution to \eqref{eq:optimal-W-MSE} is rank $d$ approximation of simplex ETF? 
    \item When $d < N$, is there a closed form solution to \eqref{eq:optimal-W-CE}? The problem reduces to Tammes problem if there is no $\exp(1)$ term and LogSumExp is equal to maximum. Tammes problem is an unsolved problem in geometry \url{http://neilsloane.com/packings/} except for particular pairs of $(K, d)$, hence we may expect not to be able to precisely characterize the solution to \eqref{eq:optimal-W-CE} as well. Nonetheless, the optimization in \eqref{eq:optimal-W-CE} provides better intuitive understanding on the property of features learned from CE loss. 
\end{itemize}

\begin{proof}
    Under Conjectures \ref{conj:within-class-collapsing} and \ref{conj:self-duality} we have
    \begin{equation}
        \W^* = \arg\min_{\W} \sum_{k=1}^K {\mc L}(\alpha\W \w_k, \y_k) + \frac{\lambda_{\W} + n^2\alpha^2\lambda_{\H}}{2} \|\W\|_F^2.
    \end{equation}
    \begin{itemize}
        \item If $\mc L$ is the MSE loss, we have
        \begin{align}
            \W^* &= \arg\min_{\W} \sum_{k=1}^K (\alpha \|\w_k\|_2^2 - 1)^2 + \sum_{k \ne k'} \alpha^2 \langle \w_k, \w_{k'} \rangle ^2 + \frac{\lambda_{\W} + n^2\alpha^2\lambda_{\H}}{2} \|\W\|_F^2\\
            &= \arg\min_{\W} \sum_{k=1}^K \left( (\alpha \|\w_k\|_2^2 - 1)^2 + \frac{\lambda_{\W} + n^2\alpha^2\lambda_{\H}}{2} \|\w_k\|_2^2\right) + \sum_{k \ne k'} \alpha^2 \langle \w_k, \w_{k'} \rangle ^2\\
            &= \arg\min_{\W} \sum_{k=1}^K \left(\alpha \|\w_k\|_2^2 + \left(\frac{\lambda_{\W}}{4\alpha} + \frac{n^2\alpha \lambda_{\H}}{4} - 1 \right) \right)^2 + \sum_{k \ne k'} \alpha^2 \langle \w_k, \w_{k'} \rangle ^2.
        \end{align}
        Using Conjecture \ref{conj:equal-norm}, we have
        \begin{equation}
            \W^* = \arg\min_{\W} \sum_{k \ne k'} \langle \w_k, \w_{k'} \rangle ^2 = \arg\min_{\W} \sum_{k \ne k'} \left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_{k'}}{\|\w_k\|_2} \right\rangle ^2
        \end{equation}

        \item If $\mc L$ is the CE loss, we have
        \begin{align}
            \W^* &= \arg\min_{\W} \sum_{k=1}^K \log\left( \frac{\sum_{k'=1}^N \exp \left(\alpha \langle \w_k, \w_k' \rangle\right)}{\exp\left(\alpha \|\w_k\|_2^2\right)}\right) + \frac{\lambda_{\W} + n^2\alpha^2\lambda_{\H}}{2} \|\W\|_F^2\\
            &= \arg\min_{\W} \sum_{k=1}^K \log\left( \sum_{k'=1}^N \exp \left(\alpha \langle \w_k, \w_k' \rangle\right)\right) - \sum_{k=1}^K \alpha \|\w_k\|_2^2 + \frac{\lambda_{\W} + n^2\alpha^2\lambda_{\H}}{2} \|\W\|_F^2\\
            &= \arg\min_{\W} \sum_{k=1}^K \log\left( \exp \left( \alpha \|\w_k\|_2^2 \right) + \sum_{k' \ne k} \exp \left(\alpha \langle \w_k, \w_k' \rangle\right)\right) + \frac{\lambda_{\W} + n^2\alpha^2\lambda_{\H} - 2\alpha}{2} \|\W\|_F^2.
        \end{align}
        Using Conjecture \ref{conj:equal-norm}, we have
        \begin{align}
            \W^* &= \arg\min_{\W} \sum_{k=1}^K \log\left( \exp\left( \alpha \beta^2 \right) + \sum_{k' \ne k} \exp \left(\alpha \langle \w_k, \w_k' \rangle\right) \right) \\
            &=  \arg\min_{\W} \sum_{k=1}^K \log\left( \exp(1) + \sum_{k' \ne k} \exp \left(\left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2} \right\rangle\right) \right)
        \end{align}
    \end{itemize}
\end{proof}




\begin{itemize}
    \item In some sense, the ideal class separation should be given by the solution to Tammes problem, as it guarantees that all pairs of classes are as sufficiently separated as possible. If so, instead of training the classifier with CE loss, can we have an approach where we first try to obtain a solution to Tammes problem, and use it as classifier weight?
    \item The case of $d <  K$ gives rise to a ``class assignment'' problem due to the reason that not all pairs of classifier weights are equal distant. To illustrate this, consider the case where there are four classes (C1 = car, C2 = truck, C3 = cat, C4 = dog) and the feature space is two-dimensional. The solution to Tammes problem is obviously given by $[1, 0], [-1, 0], [0, 1], [0, -1]$, up to rotation. Then, there are three ways of assigning classes to the weights, illustrated in Figure~\ref{fig:class-assignment}. In the first two cases, car and truck are closer, while cat and dog are closer in the feature space. In the last case, car and truck are far away, while cat and dog are also far away in the feature space. 
    
    The questions are 1) do we always obtain the same assignment if we do a standard training with CE? 2) if no to 1), is the test accuracy correlated with which assignment it converges to? 3) if yes to 1), can we fix the weight and enforce one of the two other possible assignment, and see if we can obtain a better performance? Answering such questions may shed light on developing techniques for obtaining better classification performance. \zz{do experiments with $d=2$ and the four classes: check the distribution of the classifiers.}
\end{itemize}

\begin{figure}[h]
\small
%\vspace{-5pt}
\centering
    \includegraphics[clip=true,trim=0 11cm 12cm 0,width=0.8\columnwidth]{figures/class_assignment.pdf}
    \caption{}
    \label{fig:class-assignment}
\end{figure}
% https://docs.google.com/presentation/d/1eAgj7oVeW2aH6AzcBa_bhzAPhjUtoB_6TJJsGoURJzc/edit?resourcekey=0-etyxYhH74znQyN4qLa36BA#slide=id.p




\subsection{Results on the minimum pairwise angle} 
\begin{definition}[Max-Min-Margin Classifier]
    A classifier with weight vectors $\{\u_k^* \in \Sp^{d-1}\}_{k=1}^K$ is called a maximal minimum pairwise margin classifier (\ie, a Max-Min-Margin classifier) if the minimum pairwise Euclidean distance is maximized. That is, 
    \begin{equation}
        \{\u_k^*\}_{k=1}^K = \arg\max_{\{\u_k \in \Sp^{d-1}\}_{k=1}^K} \min_{k \ne k'} \|\u_k - \u_{k'}\|_2^2,
    \end{equation}
    or equivalently,
    \begin{equation}
        \{\u_k^*\}_{k=1}^K = \arg\min_{\{\u_k \in \Sp^{d-1}\}_{k=1}^K} \max_{k \ne k'} \langle \u_k, \u_{k'}\rangle.
    \end{equation}    
\end{definition}
    \begin{equation}
        \{\w_k^*,\h_k^*\}_{k=1}^K = \arg\min_{\{\w_k,\h_k \in \Sp^{d-1}\}_{k=1}^K} \max_{k, k'} \langle \w_k, \h_{k'}\rangle.
    \end{equation}
Intuitively, a Max-Min-Margin classifier is an ideal classifier because it requires that the margin between any pairs of classes is as large as possible.
In addition, according to \Cref{thm:main}, minimizing CE is approximately maximizing the minimum pairwise angle between the rows of the weight matrix. 
Hence, in the following we first present results on properties of Max-Min-Margin Classifiers. We then discuss whether the classifiers learned under CE and MSE losses are Max-Min-Margin Classifiers.

\myparagraph{Results on max-min-margin classifier. }
We now summarize some of the existing results on the greatest value of the minimum pairwise angle. Without loss of generality and to simplify the presentation, we consider $K$ vectors $\u_1,\ldots,\u_K\in\Re^{d}$ with unit length, i.e., $\u_1,\ldots,\u_K\in\Sp^{d-1}$.




\zz{Bounds for other cases can also be found at \cite{rankin1955closest}. But it looks quite complicated.}

\myparagraph{Results for CE. }
The following result shows that minimizing a variant of the CE loss asymptotically converges to spherical uniformity. 

\begin{theorem}\cite[Theorem 3]{lu2022neural} Consider the minimization problem
\[
\min_{\u_1,\ldots,\u_K\in\Sp^{d-1} } \sum_{k=1}^K \log\left( 1 + \sum_{k'\neq k} \exp(\alpha (\langle \u_k, \u_{k'} \rangle - 1))   \right).
\]
Then for any $\alpha>0$, as $K\rightarrow \infty$, its minimizer is uniformly distributed on the sphere $\Sp^{d-1}$.
\label{eq:CE-solution-infity-K}\end{theorem}
\zz{This loss seems slightly different to CE. What about the CE loss? Similar results for other losses have also been established in the literature, e.g., \cite{liu2021learning}.}
\cy{This loss is exactly the same as \eqref{eq:optimal-W-CE} $- 1$ when $\alpha = 1$?} \zz{That's right, not sure why it has $-1$.}


For a finite $K$, we start with considering the following problem
\begin{equation}\label{eq:min-softmax-margin}
    \min_{\u_1,\ldots,\u_K\in\Sp^{d-1} } \log\left( \sum_{k' \ne k}  \exp( \langle \u_k, \u_{k'} \rangle) \right),
\end{equation}
which may be considered as a simplified version of the problem of interest in \eqref{eq:optimal-W-CE}.
\begin{proposition}
Let $\P(\U) \in \RR^ {K \times K}$ be given by
\begin{equation}
    p(\U)_{k,k'} = 
    \begin{cases}
    0, & \text{if}~k = k'\\
    \exp(\langle \u_k, \u_{k'} \rangle), & \text{otherwise.}
    \end{cases}
\end{equation}
If $\U \in \RR^{d \times K}$ is an optimal solution to \eqref{eq:min-softmax-margin} then there exists a diagonal matrix $\D \in \RR^{K \times K}$ such that $\U \cdot ( \P(\U) - \D) = 0$. 
\end{proposition}
\begin{proof}
    Computing the gradient of \eqref{eq:min-softmax-margin} w.r.t. $\U$ gives \zz{should we use the Riemannian gradient to incorporate the unit sphere constraints?}
    \begin{equation}
        \frac{\partial \log\left( \sum_{k' \ne k}  \exp( \langle \u_k, \u_{k'} \rangle)   \right)}{\partial \U} =
        \frac{\U \cdot \P(\U)}{\sum_{k \ne k'} \exp(\langle \u_k, \u_{k'} \rangle)}.
    \end{equation} 
    Let $\U^* \in \RR^{d \times K}$ be an optimal solution to \eqref{eq:min-softmax-margin}. 
    It must satisfy
    \begin{equation}
        \frac{\partial \log\left( \sum_{k' \ne k}  \exp( \langle \u_k, \u_{k'} \rangle)   \right)}{\partial \U} | _{\U = \U^*} =  \U^* \cdot \D,
    \end{equation}
    for some diagonal matrix $\D_0 \in \RR^{K \times K}$. Let $\D \doteq \left( \sum_{k \ne k'} \exp(\langle \u_k, \u_{k'} \rangle) \cdot \D_0 \right)$, and combine the two equations above, we obtain
    \begin{equation}
        \U^* \cdot \P(\U^*) = \U^* \cdot \D.
    \end{equation}

    
    \cy{Is there anything more interesting we can derive from here on relating it to max-min-margin? E.g. if $K < d$, we may check if simplex ETF satisfies this condition; it may be more difficult for $K > d$ case. Another special case is $d = 2$. }
\end{proof}
\jz{We can show that when $d=2$, feature $h_{k,i}$ are aligned with classifier weight $w_k$, and they are uniformaly distributed, under the condition that $\norm{\mb w_1}{2}=\norm{\mb w_2}{2}=\cdots=\norm{\mb w_k}{2}$.}

\begin{proof}
    Let $\mb W = 
    \begin{bmatrix} 
        \mb w_1 & \cdots & \mb w_K 
    \end{bmatrix}^\top \in \bb R^{K \times d}$, $\mb H = \begin{bmatrix}
    \mb h_1 & \mb h_2 & \cdots & \mb h_K
    \end{bmatrix}\in \bb R^{d \times K}$, and $\norm{\mb w_1}{2}=\norm{\mb w_2}{2}=\cdots=\norm{\mb w_k}{2}=1$. 
    \begin{align*}
        {\mc L}_{ce} (\mb W\mb H) &= -\frac{1}{K}\sum\limits_{k=1}^K\log\paren{\frac{\exp{(\mb w_k^\top \mb h_k)}}{\sum\limits_{j=1}^K \exp{(\mb w_j^\top \mb h_k)}}}\\
        &= \frac{1}{K}\sum\limits_{k=1}^K\log\paren{1+\sum_{j \neq k}^K\exp{\paren{(\mb w_j - \mb w_k)^\top\mb h_k}}}
    \end{align*}
    for cross-entropy loss, we can consider each sample individually, for any sample k, we have:
    \begin{align*}
        {\mc L}_{ce} (\mb W\mb h_k) &= \log\paren{1+\sum_{j \neq k}^K\exp{\paren{(\mb w_j - \mb w_k)^\top\mb h_k}}}
    \end{align*}
    for the consistence, let denote $\mb w_K = \mb w_0 = \mb w_{-K},  \mb w_{K+1} = \mb w_1=\mb w_{-K+1} \cdots, \mb w_{K+K-1} = \mb w_{K-1} = \mb w_{-1}$. Then, we can find the lower bound for sample k as following:
    \begin{align}
        {\mc L}_{ce} (\mb W^*\mb h_k^*) &= \log\paren{1+\sum_{j \neq 1}^K\exp{\paren{(\mb w_j^* - \mb w_k^*)^\top\mb h_k^*}}} \nonumber\\
        &= \log\paren{1+\sum_{j =1}^{K-1}\frac{\exp{\paren{(\mb w^*_{k-j} - \mb w_k^*)^\top\mb h_k^*}}+\exp{\paren{(\mb w^*_{k+j} - \mb w_k^*)^\top\mb h_k}}}{2}} \nonumber\\
        &\geq \log\paren{1+\sum_{j =1}^{K-1}\exp{\paren{\paren{\frac{\vw^*_{k-j}+\vw^*_{k+j}}{2}-\vw_k^*}^\top\vh_k^*}}}
    \end{align}
    
    The inequality holds only when $(\mb w_{k-j} - \mb w_k)^\top\mb h_k = (\mb w_{k+j} - \mb w_k)^\top\mb h_k$, which means $(\vw_{k-j}-\vw_{k+j})^\top\vh_k=0$, for $j = 1,\cdots, K-1$. Since $\norm{\vw_1}{2}=\cdots=\norm{\vw_K}{2}=1$, we can have $\vh_k\parallel (\vw_{k-j}+\vw_{k+j})$. Denote $\vh_k = \pm\norm{\vh_k}{2} \frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}$, we can have following:
    \begin{itemize}
     \item{ if $\vh_k = \norm{\vh_k}{2} \frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}$:}
     \begin{align}
        \paren{\frac{\vw_{k-j}+\vw_{k+j}}{2}-\vw_k}^\top\vh_k &= \norm{\vh_k}{2}\paren{\frac{\vw_{k-j}+\vw_{k+j}}{2}-\vw_k}^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}\nonumber\\
        &=\norm{\vh_k}{2}\paren{\frac{\norm{\vw_{k-j}+\vw_{k+j}}{2}}{2}-\vw_k^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}}\nonumber\\
        &= \norm{\vh_k}{2}\paren{\frac{\norm{\vw_{k-j}+\vw_{k+j}}{2}\norm{\vw_k}{2}}{2}-\vw_k^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}}\nonumber\\
        &\geq \norm{\vh_k}{2}\paren{\frac{\vw_k^\top(\vw_{k-j}+\vw_{k+j})}{2}-\vw_k^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}}\nonumber
    \end{align}
    where the inequality achieves equality only when $\vw_k=\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}$, and for $-\vw_k^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}$, it also achieves minimum when $\vw_k=\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}$. Therefore, $\vh_k=\norm{\vh_k}{2}\vw_k$.
    \item{ if $\vh_k = -\norm{\vh_k}{2} \frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}$:}
     \begin{align}
        \paren{\frac{\vw_{k-j}+\vw_{k+j}}{2}-\vw_k}^\top\vh_k &= -\norm{\vh_k}{2}\paren{\frac{\vw_{k-j}+\vw_{k+j}}{2}-\vw_k}^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}\nonumber\\
        &=-\norm{\vh_k}{2}\paren{\frac{\norm{\vw_{k-j}+\vw_{k+j}}{2}}{2}-\vw_k^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}}\nonumber\\
        &= -\norm{\vh_k}{2}\paren{\frac{\norm{\vw_{k-j}+\vw_{k+j}}{2}\norm{\vw_k}{2}}{2}-\vw_k^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}}\nonumber\\
        &\geq -\norm{\vh_k}{2}\paren{-\frac{\vw_k^\top(\vw_{k-j}+\vw_{k+j})}{2}-\vw_k^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}}\nonumber\\
        &=\norm{\vh_k}{2}\paren{\frac{\vw_k^\top(\vw_{k-j}+\vw_{k+j})}{2}+\vw_k^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}}\nonumber
    \end{align}
    where the inequality achieves equality only when $\vw_k=-\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}$, and for $\vw_k^\top\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}$, it achieves minimum when $\vw_k=-\frac{\vw_{k-j}+\vw_{k+j}}{\norm{\vw_{k-j}+\vw_{k+j}}{2}}$. Therefore, $\vh_k=\norm{\vh_k}{2}\vw_k$ also holds.
    \end{itemize}
    In conclusion, we have complete the proof for $\vh_k=\norm{\vh_k}{2} w_k$ for $k=1,\cdots, K$. And since $(\mb w_{k+j} - \mb w_{k-j})^\top\vw_k=0$, for $j = 1,\cdots, K-1$, and $\norm{\vw_1}{2}=\cdots = \norm{\vw_K}{2}=1$, therefore, $w_1, \cdots, \w_K$ are either uniformaly distributed, or $\vw_1= \cdots=\w_K$. \jz{Is there some previous work to formally prove this argument? I verify this results for $K=5$.}
    
    \jz{denote $l_k=\norm{\vh_k}{2}$, next step: to show ${\hat{\mc L}}_{ce} (l_k) = \log\paren{1+\sum\limits_{j =1}^{\lfloor \frac{K}{2}\rfloor}\exp{(l_k(\cos{\frac{j\pi}{K}}-1)})}+\lambda_{\mH}l_k^2$ has unique solution $l_k^\star$ for any $\lambda_{\mH}$. As shown in \ref{fig:example-illustration}, it seems to have unique solution $l_k^\star$ for different K. As K increases, the $l_k^\star$ increases and the neighbor around $l_k^\star$ becomes more flat.}
\end{proof}
\begin{figure}[h]
\small
%\vspace{-5pt}
\centering
    \includegraphics[width=0.6\columnwidth]{figures/example.png}
    \caption{}
    \label{fig:example-illustration}
\end{figure}

\begin{theorem} Consider the objective in \eqref{eq:optimal-W-CE}
\begin{equation}
    f(\W) \doteq \sum_{k=1}^K \log\left( \exp(1) + \sum_{k' \ne k} \exp \left(\left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2}. \right\rangle\right) \right).
\end{equation}
If $K \le d+1$, then $f(\W) \ge g(K)$ for some function $g(K)$, and the equality is only achieved when $\{\w_1,\ldots,\w_K\}$ is a simplex ETF. 
\end{theorem}


Denote $v_{k, k'} \doteq \left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2} \right\rangle$. 
By Jensen's inequality, for any $k \in [K]$ we have
\begin{equation}
    \sum_{k' \ne k} \exp \left(v_{k, k'}\right) \ge (K-1) \exp  \left( \frac{\sum_{k' \ne k} v_{k, k'}}{K-1} \right).
\end{equation}
where the equality holds if and only if $v_{k, k'}$ is independent of $k'$. By further using the following Jensen's inequality
\begin{equation}
    \log \frac{a_1 x_1 + a_2 x_2}{a_1 + a_2} \ge \frac{a_1 \log x_1 + a_2 \log x_2}{a_1 + a_2},
\end{equation}
where we take 
\begin{gather}
    a_1 = \frac{1}{K-1} \exp(\frac{1}{K-1}), x_1 = (K-1) \exp\left(\frac{K - 2}{K-1}\right), \\
    a_2 = \exp(-1), x_2 = (K-1) \exp\left(\frac{\sum_{k' \ne k} v_{k, k'}}{K-1} + 1\right), 
\end{gather}
we obtain
\begin{multline}
    \log \left(\exp(1) + (K-1) \exp  \left( \frac{\sum_{k' \ne k} v_{k, k'}}{K-1} \right) \right)
    \ge \log \left( \frac{1}{K-1} \exp(\frac{1}{K-1}) + \exp(-1) \right) + \\
    \frac{ \frac{1}{K-1} \exp(\frac{1}{K-1}) (\log (K-1) + \frac{K - 2}{K-1}) + \exp(-1) \log(K-1) + \exp(-1) \left(\frac{\sum_{k' \ne k} v_{k, k'}}{K-1} - 1\right)}{ \frac{1}{K-1} \exp(\frac{1}{K-1}) + \exp(-1) } \doteq A \sum_{k' \ne k} v_{k, k'} + C,
\end{multline}
where $A > 0, C$ are functions of $K$. 
The inequality holds if and only if $x_1 = x_2$, that is, when
\begin{equation}
    (K-1) \exp\left(\frac{K - 2}{K-1}\right) = (K-1) \exp\left(\frac{\sum_{k' \ne k} v_{k, k'}}{K-1} + 1\right) 
    \iff 
    \sum_{k' \ne k} v_{k, k'} = -1.
\end{equation}
Combining the two inequalities above we obtain
\begin{equation}
    f(\W) \ge A \sum_{k=1}^K \sum_{k' \ne k} v_{k, k'} + C \cdot K 
    = A \sum_{k, k'} v_{k, k'} + (C - A) \cdot K 
    = A \norm{\sum_{k=1}^K \frac{\w_k}{\|\w_k\|_2}}{2}^2 + (C - A) \cdot K \ge (C - A) \cdot K,
\end{equation}
where the last inequality holds if and only if $\sum_{k=1}^K \frac{\w_k}{\|\w_k\|_2} = 0$.
Combining above, we have $f(\W) \ge (C - A) K$ with equality holds if and only if $\sum_{k=1}^K \frac{\w_k}{\|\w_k\|_2} = 0$ and $\left\langle \frac{\w_k}{\|\w_k\|_2}, \frac{\w_k'}{\|\w_{k'}\|_2} \right\rangle = -\frac{1}{K-1}$ for all pairs of $k, k'$.


\myparagraph{Results for MSE. }

\begin{theorem}[MSE leads to orthogonal vectors] Assume $K \le d$. Then
\[
\sum_{k\neq k'} \langle \u_k, \u_{k'} \rangle^2 \ge 0,
\]
always holds, and the equality is achieved if e.g., $\U = [I; 0]$.
\end{theorem}
\begin{proof}
    The lower bound of $0$ is obvious since each term in the summation is nonnegative. The solution $\U = [I; 0]$ achieves this lower bound is easy to verify. Conjecture: by following the proof technique in the next Thm, we can show that the equally holds if and only if $\U^\top \U = I$.
\end{proof}
\cy{This result seems strange as it is not a simplex ETF, hence inconsistent to known results for MSE loss. It may be due to the self-duality conjecture. } \zz{For MSE loss, we have simplex ETF if we have the bias. Without this bias term, the solutions become orthonormal matrices.}

The following result characterizes the solutions for minimizing the mean squared pairwise angles. 
\begin{theorem}[MSE leads to tight frame] Assume $K \ge d$. Then
\[
\sum_{k\neq k'} \langle \u_k, \u_{k'} \rangle^2 \ge \frac{K^2 - Kd}{d}
\]
always holds, and the equality is achieved only when $\U = \begin{bmatrix}\u_1 & \cdots & \u_K \end{bmatrix}$ forms a unit-norm tight frame (UNTF), i.e., $\U \U^\top = \frac{K}{d} I_d$. %\cy{Should it be $\U \U^\top = K/d I_d$, since $\sigma_i = K/d$?}
\end{theorem}
\begin{proof} Let $\sigma_1 \ge \sigma_2 \cdots \ge \sigma_d$ be the $d$ largest eigenvalues of $\U^\top \U$. The rest of the eigenvalues of  $\U^\top \U$ are zero since $\U^\top \U$ has rank at most $d$. First note that
\[
\sum_{i=1}^d \sigma_i = \trace(\U^\top \U) = K.
\]
On the other hand, 
\[
\norm{\U^\top \U}{F}^2 = K + \sum_{k \neq k'} \langle \u_k, \u_{k'}\rangle^2 = \sum_{i=1}^d \sigma_i^2 \ge \frac{1}{d} \left( \sum_{i=1}^d \sigma_i \right)^2 = \frac{K^2}{d},
\]
which further implies that 
\[
\sum_{k\neq k'} \langle \u_k, \u_{k'} \rangle^2 \ge \frac{K^2 - Kd}{d}.
\]
The inequality becomes equality when $\sum_{i=1}^d \sigma_i^2 = \frac{1}{d} \left( \sum_{i=1}^d \sigma_i \right)^2$, which holds only when $\sigma_1 = \cdots = \sigma_d = \frac{K}{d}$.
\end{proof}

Minimizing the mean squared pairwise angles has been extensively studied in the tight-frame literature, where  $\sum_{k}\sum_{k'} \langle \u_k, \u_{k'} \rangle^2 $ is called the {\it frame potential} \cite{waldron2018introduction}. The work showed that the problem of minimizing frame potential over $\u_1,\ldots,\u_K\in\Sp^{d-1}$ has no spurious local minima, i.e., any local minimizer must be a UNTF
\cite{benedetto2003finite}. The work 
\cite{goyal2001quantized,zimmermann2001normalized} showed the existence of UNTFs for any $d$ and $K\ge d$. Finally, we note that minimizing  mean squared pairwise angles may not lead to a solution with uniformly distributed unit vectors on the sphere \cy{uniformly is not defined? we may switch to using max-min-margin classifier notion}, as implied by the following example.

\begin{example}[UNTFs with non-uniformly distributed vectors] For and $d$, suppose $K = m d$ with any positive integer $m$. Let $\O_d \in \Re^{d\times d}$ be any orthonormal matrix. Then $\U = \underbrace{\begin{bmatrix} \O_d & \O_d & \cdots & \O_d \end{bmatrix}}_{m \text{ times}} \in \Re^{d\times K}$ is a UNTF with $K$ unit vectors since $\U \U^\top = m \O_d \O_d^\top = m I_d$. Hence, it is also a global minimizer of the frame potential, or $\sum_{k\neq k'} \langle \u_k, \u_{k'}\rangle^2$. 
\end{example}

\cy{We can also consider if the following is true: there always exist a UNTF that is a MMM classifier.} \zz{seems there exist cases when a MMM classifier is not a UNTF.}


When $K\ge d$, the max-min-margin classifier, i.e., the Tammes' problem,  turns out to be extremely difficult. Even when $d = 3$, the exact solutions to this problem are  known only for limited cases, such as $K = 3,4,\ldots,12$ and $K =24$. \zz{more solutions founded recently?} Among these settings, according to \cite{fickus2001finite}, the solutions for $K = 4,6$ are UNTF, but the solution for $K = 5$ is not a UNTF. Moreover, there appears to be a growing distinction between the solutions of Tammes' problem and UNTFs when $K\ge 7$ becomes larger. \zz{be careful about the last sentence.}


\begin{theorem}\cite{goyal1998quantized} Let $\{\u_k\}$ be independently selected from a uniform distribution on the sphere in $\Re^d$. Then the matrix $\U_K = \begin{bmatrix} \u_1 & \cdots & \u_K
\end{bmatrix}$ converges to a UNTF when $K$ goes to infinity in the sense that 
\[
\frac{1}{K} \U_K \U_K^\top \Longrightarrow \frac{1}{d}I_d \quad \textup{elementwise as}\quad K \rightarrow \infty.
\]

\end{theorem}
\zz{\Cref{eq:CE-solution-infity-K} shows that the solution for CE converges to spherical uniformity when $K\rightarrow\infty$. Does this mean that the solution for CE converges to a UNFT when $K\rightarrow\infty$? Is the notion of spherical uniformity different to independently sampling from a uniform distribution?}


\subsection{The blessing of dimensionality}

In applications like face classification and self-supervised learning where each training sample is viewed as an individual class, the number of classes (e.g., millions of classes)  could be significantly larger than the dimensionality of the features (e.g., feature dimension is 512). Why good performance is still achieved in this case? We provide a justification through the property of high dimensionality, which is often known as the curse of dimensionality but is referred to as the blessing of dimensionality here as the classes are easily separated in high dimensions. We can explain this from the following two perspectives. First, the number of vectors in $\Re^d$ that are almost orthogonal increases exponentially in terms of $d$, i.e., there are $\exp(d)$ number of vectors in $\Re^d$ that are almost orthogonal.  \zz{Add a rigorous argument by generating random vectors and studying the pairwise angles.} Second, when $K$ vectors $\{\u_1,\ldots,\u_K\}$ in $\Re^d$ are properly placed, the maximal pair-wise angle satisfies $
\max_{k\neq k'} \langle \u_k, \u_{k'} \rangle \lesssim \frac{\log K}{d}$ \zz{do we have such a result?} \zz{Also run experiments to show the minimal pair-wise angle found by CE loss for different pairs of $d$ and $K$.}

\section{Theoretical Analysis}



\section{The assignment problem}


\section{Experiments}
\zz{Experiments:
\begin{itemize}
\item Verify NC1, NC2, and tight frame
\item Design loss: compare MSE, CE, and new loss that better approximates Max-min-margin classifier?
\item Assignment - observe whether 1) the assignment of classes to MMM classifier weights are consistent across independent trials, 2) different assignment leads to different test performance (or if there is a one-to-one correspondence between them).
\item Set the classifier initialization as the class-mean features? or adjust the classifier based on the class-mean features.
\end{itemize}
}

\jz{ experiments links ~\url{https://docs.google.com/presentation/d/1BkYoFsc27MIgng5b7wbe_E5jSP7YTe1LePTEtsc4gPY/edit#slide=id.p}}

Aside from the three NC properties, we can also check another property, the tight frame for the class-mean features $\overline \H^*$ or the classifiers $\W^{*\top}$, i.e., $ \overline \H^* \overline \H^{*\top} = \alpha \W^{*\top} \W^{*} = \beta I_d$. This can be measured by 
\[
\norm{ \frac{ \W^{*\top} \W^{*}}{\norm{\W^{*\top} \W^{*}}{F}}  -  \frac{1}{\sqrt{d}}I_d}{F}
\]
or the variance of the singular values of $\W^{*\top}$: suppose $\sigma_1,\ldots, \sigma_d$ are the $d$ singular values (with $K\ge d+1$), 

\subsection{Effect of feature dimension}

\begin{table}[]
    \centering
    \begin{tabular}{c|ccccccc}
        Dim & 8 & 16 & 32 & 64 & 128 & 512 & 1024  \\
        \midrule
        Train Acc & 68.66 & 73.60 & 76.22 & 78.25 & 80.04 & 82.05 & 82.07 \\
        Eval Acc & 70.45 & 72.99 & 73.89 & 74.62 & 74.89 & 75.47 & 75.34 \\
    \end{tabular}
    \caption{Performance of ResNet-50 with varying feature dimensions for ImageNet classification. In a standard ResNet-50, the output from the last residual block is mapped to $1000$ dimensional logit space through a linear layer. Here to control the dimension of the feature space, we first project the output of the last residual block into a $d$-dimensional feature space through a linear layer, before mapping it into the $1000$ dimensional logit space.}
    \label{tab:feature-dim-imagenet}
\end{table}
